GPT-4V(ision) is a Generalist Web Agent, if Grounded

The recent development on large multimodal models (LMMs), especially GPT-4V(ision) and Gemini, has been quickly expanding the capability boundaries of multimodal models beyond traditional tasks like image captioning and visual question answering. In this work, we explore the potential of LMMs like GPT-4V as a generalist web agent that can follow natural language instructions to complete tasks on any given website. We propose SEEACT, a generalist web agent that harnesses the power of LMMs for integrated visual understanding and acting on the web. We evaluate on the recent MIND2WEB benchmark. In addition to standard offline evaluation on cached websites, we enable a new online evaluation setting by developing a tool that allows running web agents on live websites. We show that GPT-4V presents a great potential for web agents -- it can successfully complete 51.1 of the tasks on live websites if we manually ground its textual plans into actions on the websites. This substantially outperforms text-only LLMs like GPT-4 or smaller models (FLAN-T5 and BLIP-2) specifically fine-tuned for web agents. However, grounding still remains a major challenge. Existing LMM grounding strategies like set-of-mark prompting turns out to be not effective for web agents, and the best grounding strategy we develop in this paper leverages both the HTML structure and visuals. Yet, there is still a substantial gap with oracle grounding, leaving ample room for further improvement. All code, data, and evaluation tools are available at https://github.com/OSU-NLP-Group/SeeAct.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
\begin{abstract}
The advancement of autonomous web navigation has faced obstacles due to the complexity of web environment. Vision Language Models have shown impressive ability in image understanding, which suggests it has great potential to enhance web navigation tasks. However, there hasn't been a comprehensive quantitative performance assessment of the model for this task. In this work, we delve into the effectiveness of GPT-4V(vision) in web navigation tasks, with a particular focus on its ability to describe and accurately reference specific webpage elements. The main contributions of our study are two-fold. Firstly, we conduct a thorough assessment of GPT-4V's performance in web navigation through human evaluation. This investigation not only benchmarks the model's current capabilities but also sets a foundation for understanding its practical applications and limitations in real-world web agents. Addressing the limitation of referring in GPT-4V\jh{what kind of limitations? Perhaps explain it a bit more?}, we propose and detail three solutions. These strategies are designed to enhance the model's accuracy in referring to webpage elements, tackling the issue through element attribute identification, text-based candidate, and image annotation.\jh{a bit confused about what the three solutions exactly are. Perhaps, adding Roman Numerals to each solution (\eg, (i), (ii), (iii)).}  Our findings not only demonstrate GPT-4V's potential in web navigation tasks but also suggest the bottleneck in image detail referring.
\jh{where is the 2nd fold? looks like I can only see the 1st fold.}

\boyuan{Add Conclusions and some take-away messages}
\end{abstract}

==> sec/1_intro_v2.tex <==
\section{Introduction}
\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics[width=1\linewidth]{figs/teaser_fig.pdf}
    }
    \caption{
    GPT4 grounds to the web environment with the lengthy HTML text as shown on the left. With HTML text, the referring won't be too hard, the model can directly generate the element node id. 
    GPT-4V grounds to the web environment through a webpage screenshot, which serves as a better representation with more condensed information. The image detail referring will be more challenging than text-only model.
    % A segment of a webpage screenshot corresponds to a significant amount of tokens for its HTML text counterpart, even when CSS is excluded. 
    \boyuan{[TODO: Will simplify the teaser figure]}
    }
    \label{fig:teaser}
    %\vspace{-15pt}
\end{figure}

- importance of web agents, earlier datasets, mind2web
- primarily text-based LLMs. while some recent work on VLM (Pix2Act, WebGUM), they are primarily use small models. what's the disadvanges? 

Recent advancements in Vision Language Models (VLMs) have marked a significant leap forward in multimodal scenarios~\cite{Li2023MultimodalFM, yang2023dawn}
\hs{should cite more work}. 
Emerging research is increasingly leveraging image representations to empower web navigation tasks~\cite{Li2022SpotlightMU, Shaw2023FromPT, Furuta2023MultimodalWN}\hs{are they already doing web navigation, the same thing as we are? are you implying they'll be our baselines? if not, then rephrase this?}. 
Unlike text-only models that can only ground on HTML text within limited token length, VLMs leverage condensed, visual-rich image representations, preserving crucial visual cues and facilitating more nuanced web agent interactions.\jh{w/ this sentence, not sure how the image can help more. Perhaps give some real examples?} As the old saying goes, ``a picture is worth a thousand words'': A small segment of a webpage image can encapsulate what tens of thousands of HTML tokens convey. 
% As illustrated in Figure~\ref{fig:teaser}, a screenshot segment worthing merely \num{595}~\footnote{Calculated with OpenAI Vision pricing calculator: \url{https://openai.com/pricing}} text tokens\hs{I don't quite get what this means.} needs \num{43215} HTML tokens to convey its meaning.



% Webpage image shows several advantages as the representation to ground web agent comparing with HTML text: (1) Efficient Representation: Images provide a condensed, information-rich format that circumvents the verbosity and context limitations inherent in extensive HTML texts. (2) Preservation of Visual Information: Crucial visual information is retained, enhancing comprehension and interpretation. (3) Enhanced Webpage Interaction: Designed for human engagement, webpage environments convey a wealth of actionable data, beneficial for web agents in decision-making processes. As shown in Figure~\ref{fig:teaser}, even a small chunk in the webpage screenshot image corresponds to a lengthy HTML text with 43,215 tokens even after removing all CSS codes for visual features. However, the corresponding image screenshot only need 595~\footnote{Approximation via OpenAI \href{https://openai.com/pricing}{Vision pricing calculator}} text token after projecting the corresponding image. 

Fine-tuning VLMs on annotated datasets has shown promise for web navigation and mobile UI comprehension, as demonstrated by WebAgent~\cite{Gur2023ARW}, WebGUM~\cite{Furuta2023MultimodalWN}, and Pix2Act~\cite{Shaw2023FromPT}. Despite their potential, these models often struggle with generalizing to new, unseen distributions\hs{environments?}. In contrast, foundation models such as LLaVa~\cite{Liu2023VisualIT} and MiniGPT4~\cite{Zhu2023MiniGPT4EV}, Bard-Vision offer better generalization but fall short in complex web navigation tasks.\jh{Perhaps, show some examples/results supporting this claim: fine-tuned models are less generalizable than foundation models?}

The advent of the GPT-4V model brings new excitement to the field. While many works \cite{Yan2023GPT4VIW, cui2023holistic, Yang2023SetofMarkPU, Wen2023OnTR, Yang2023Idea2ImgIS, Lin2023MMVIDAV} have already shown their strong capabilities in a wide range of tasks and scenarios, its potential for the web scenario is still under-explored. 

\boyuan{[Pulled from Online Evaluation Section]}




% \boyu{"Previous is not golden, have to fix the error it self.so it needs to fix its error. and it's an exploration. which is a good point."}

Besides web agent modeling, evaluation is also a major challenge here, despite substantial efforts to develop such an ideal benchmark. Webshop~\cite{Yao2022WebShopTS}, miniWoB++\cite{liu2018reinforcement}, and WebArena\cite{Zhou2023WebArenaAR} create local website environments to facilitate dynamic interactions. However, the engineering work required to build these web environments is extensive, leading to a limited number of websites and insufficient task diversity. The simulated environments are also not close enough to real websites. An ideal benchmark should be diverse enough with numerous websites, tasks across numerous domains and can provide dynamic interaction with the web agent. Although signiciant efforts has been invested in building benchmarks, they are far from a ideal benchmark. Dynamic benchmarks, like WebArena, can support interaction with web agents, but fall short in environment diversity and resemblence to real websites. In contrast, offline benchmarks, like Mind2Web, has the advantage of diversity, but can not support dynamic interaction and feedback for agents.

Step-wise performance provides a good evaluation of the models' ability to ground to web environments and generate a single action. However, these evaluation is not enough to assess agents' ability to complete whole tasks on websites. An ideal benchmark should possess the following properties: (1) Broad coverage of diverse website environments across various domains; (2) Diverse tasks that can challenge multiple aspects of the model's capability; (3) Dynamic environment to allow various action paths and provide interactions and feedbacks to agents.



Mind2Web~\cite{deng2023mind2web} fulfills the first two criteria by dumping webpages from numerous websites across a wide range of domains and annotating a large set of diverse tasks with annotated traces. However, Mind2Web only offers an offline environment through webpage dumps. This offline approach has two primary limitations:
\begin{itemize}
\item \textbf{Action Sequence Variability} A single task can be completed through multiple potential action sequences, such as altering the order of actions, as depicted in Figure~\ref{fig:online-eval}. In an offline environment, evaluations can only compare the generated action sequence with a single predefined target sequence.
\item \textbf{Lack of Environment Interaction} Interactions with the environment are critical for web agents to correct errors and explore options to find the optimal solution, as illustrated in Figure~\ref{fig:online-eval}. Offline environments lack this interactive component.
\end{itemize}

\boyuan{[Will rewrite the online evaluation section in intro]}

This paper fills the gap with the following contributions: 
\begin{itemize}
    \item We investigate GPT-4V's proficiency in web navigation, by presenting the first quantitative analysis and establishing a performance benchmark via human evaluation. \boyu{Boyu: Is it okay to say we established a benchmark?}
    \item We pinpoint the challenges associated with webpage element referencing and propose three solutions underpinned by experimental findings and a comprehensive analysis of their strengths and limitations. With the referring techniques, GPT-4V based agents achieve superior performance on the popular Mind2Web benchmark.\jh{what are the three solutions?} 
    \item %We introduce a novel online evaluation framework for web agents, enabling real-time performance assessments on live websites, thus overcoming the constraints of traditional simulated evaluations.
    To address the limitations of using offline, offline datasets for evaluating task completion\hs{I feel the contribution of this online evaluation framework is understated; it is not just to address the limitation of `offline datasets', it also addresses the limitation of using WebArena-kind of datasets which are dynamic, but limited in scope.}, we propose a novel online evaluation framework on real, live websites. This enables real-time assessment and addresses the shortcomings of offline environments.\jh{Not sure what the online evaluation framework looks like. Perhaps explain more details about the framework?}
\end{itemize}

\nop{Additionally, we explore the limitations of using offline datasets for evaluating task completion and propose a novel, live evaluation framework on actual websites. This allows for real-time assessment and addresses the shortcomings of offline simulated environments in Mind2Web. \boyuan{[add some conclusion]}

To summarize, our contributions are threefold:
\begin{itemize}
    \item We present the first quantitative analysis of GPT-4V in web navigation, establishing a performance benchmark via human evaluations.
    \item We pinpoint the challenges associated with webpage element referencing and propose three solutions underpinned by experimental findings and a comprehensive analysis of their strengths and limitations. With proper referring, our web agent based on GPT-4V achieves the best performance on Mind2Web.
    \item We introduce a novel online evaluation framework for web agents, enabling real-time performance assessments on live websites, thus overcoming the constraints of traditional simulated evaluations.
\end{itemize}
}

==> sec/1_intro_v3.tex <==
\section{Introduction}
\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics[width=1\linewidth]{figs/teaser_v4.pdf}
    }
    \caption{
    GPT4 grounds to the web environment with the lengthy HTML text as shown on the left. With HTML text, the referring won't be too hard, the model can directly generate the element node id. 
    GPT-4V grounds to the web environment through a webpage screenshot, which serves as a better representation with more condensed information. The image detail referring will be more challenging than text-only model.
    % A segment of a webpage screenshot corresponds to a significant amount of tokens for its HTML text counterpart, even when CSS is excluded.
    }
    \label{fig:teaser}
    %\vspace{-15pt}
\end{figure}

- importance of web agents, earlier datasets, mind2web
- primarily text-based LLMs. while some recent work on VLM (Pix2Act, WebGUM), they are primarily use small models. what's the disadvanges? 

Recent advancements in Vision Language Models (VLMs) have marked a significant leap forward in multimodal scenarios~\cite{Li2023MultimodalFM, yang2023dawn}
\hs{should cite more work}. 
Emerging research is increasingly leveraging image representations to empower web navigation tasks~\cite{Li2022SpotlightMU, Shaw2023FromPT, Furuta2023MultimodalWN}\hs{are they already doing web navigation, the same thing as we are? are you implying they'll be our baselines? if not, then rephrase this?}. 
Unlike text-only models that can only ground on HTML text within limited token length, VLMs leverage condensed, visual-rich image representations, preserving crucial visual cues and facilitating more nuanced web agent interactions.\jh{w/ this sentence, not sure how the image can help more. Perhaps give some real examples?} As the old saying goes, ``a picture is worth a thousand words'': A small segment of a webpage image can encapsulate what thousands of HTML tokens attempt to convey. 
% As illustrated in Figure~\ref{fig:teaser}, a screenshot segment worthing merely \num{595}~\footnote{Calculated with OpenAI Vision pricing calculator: \url{https://openai.com/pricing}} text tokens\hs{I don't quite get what this means.} needs \num{43215} HTML tokens to convey its meaning.



% Webpage image shows several advantages as the representation to ground web agent comparing with HTML text: (1) Efficient Representation: Images provide a condensed, information-rich format that circumvents the verbosity and context limitations inherent in extensive HTML texts. (2) Preservation of Visual Information: Crucial visual information is retained, enhancing comprehension and interpretation. (3) Enhanced Webpage Interaction: Designed for human engagement, webpage environments convey a wealth of actionable data, beneficial for web agents in decision-making processes. As shown in Figure~\ref{fig:teaser}, even a small chunk in the webpage screenshot image corresponds to a lengthy HTML text with 43,215 tokens even after removing all CSS codes for visual features. However, the corresponding image screenshot only need 595~\footnote{Approximation via OpenAI \href{https://openai.com/pricing}{Vision pricing calculator}} text token after projecting the corresponding image. 

Fine-tuning VLMs on annotated datasets has shown promise for web navigation and mobile UI comprehension, as demonstrated by WebAgent~\cite{Gur2023ARW}, WebGUM~\cite{Furuta2023MultimodalWN}, and Pix2Act~\cite{Shaw2023FromPT}. Despite their potential, these models often struggle with generalizing to new, unseen distributions\hs{environments?}. In contrast, foundation models such as LLaVa~\cite{Liu2023VisualIT} and MiniGPT4~\cite{Zhu2023MiniGPT4EV}, Bard-Vision offer better generalization but fall short in complex web navigation tasks.\jh{Perhaps, show some examples/results supporting this claim: fine-tuned models are less generalizable than foundation models?}

The advent of the GPT-4V model brings new excitement to the field. While many works \cite{Yan2023GPT4VIW, cui2023holistic, Yang2023SetofMarkPU, Wen2023OnTR, Yang2023Idea2ImgIS, Lin2023MMVIDAV} have already shown their strong capabilities in a wide range of tasks and scenarios, its potential for web navigation is still under-explored. 

\boyuan{[Pulled from Online Evaluation Section]}

Besides web agent modeling, evaluation is also a major challenge here, despite substantial efforts to develop such an ideal benchmark. Webshop~\cite{Yao2022WebShopTS}, miniWoB++\cite{liu2018reinforcement}, and WebArena\cite{Zhou2023WebArenaAR} create local website environments to facilitate dynamic interactions. However, the engineering work required to build these web environments is extensive, leading to a limited number of websites and insufficient task diversity. The simulated environments are also not close enough to real websites. An ideal benchmark should be diverse enough with numerous websites, tasks across numerous domains and can provide dynamic interaction with the web agent. Although signiciant efforts has been invested in building benchmarks, they are far from a ideal benchmark. Dynamic benchmarks, like WebArena, can support interaction with web agent, but fall short in environment diversity and resemblence to real websites. In contrast, static benchmarks, like Mind2Web, has the advantage of diversity, but can not support interaction with agents.

Step-wise performance provides a good evaluation of the models' ability to ground to web environments and generate a single action. However, these evaluation is not enough to assess agents' ability to complete whole tasks on websites. An ideal benchmark should possess the following properties: (1) Broad coverage of diverse website environments across various domains; (2) Diverse tasks that can challenge multiple aspects of the model's capability; (3) Dynamic environment to handle action sequence variability and provide interactions and feedbacks to agents.

Mind2Web~\cite{deng2023mind2web} fulfills the first two criteria by dumping webpages from numerous websites across a wide range of domains and annotating a large set of diverse tasks with annotated traces. However, Mind2Web only offers a static environment through webpage dumps. This static approach has two primary limitations:
\begin{itemize}
\item \textbf{Action Sequence Variability} A single task can be completed through multiple potential action sequences, such as altering the order of actions, as depicted in Figure~\ref{fig:online-eval}. In a static environment, evaluations can only compare the generated action sequence with a single predefined target sequence.
\item \textbf{Lack of Environment Interaction} Interactions with the environment are critical for web agents to correct errors and explore options to find the optimal solution, as illustrated in Figure~\ref{fig:online-eval}. Static environments lack this interactive component.
\end{itemize}

% \boyu{Boyu's comment: Do you really want to leave all the comparison of Offline VS online in the Intro?}

% \boyuan{[Will rewrite the online evaluation section in intro]}

This paper fills the gap with the following contributions: 
\begin{itemize}
    \item We investigate GPT-4V's proficiency in web navigation, by presenting the first quantitative analysis and establishing a performance benchmark via human evaluation.
    \item We pinpoint the challenges associated with webpage element referencing and propose three novel solutions underpinned by experimental findings and a comprehensive analysis of their strengths and limitations. With our optimized referencing techniques, GPT-4V based agents achieve superior performance on the popular Mind2Web benchmark.\jh{what are the three solutions?}
    \item %We introduce a novel online evaluation framework for web agents, enabling real-time performance assessments on live websites, thus overcoming the constraints of traditional simulated evaluations.
    To address the limitations of using offline, static datasets for evaluating task completion\hs{I feel the contribution of this online evaluation framework is understated; it is not just to address the limitation of `offline, static datasets', it also addresses the limitation of using WebArena-kind of datasets which are dynamic, but limited in scope.}, we propose a novel online evaluation framework on real, live websites. This enables real-time assessment and addresses the shortcomings of static environments.\jh{Not sure what the online evaluation framework looks like. Perhaps explain more details about the framework?}
\end{itemize}

\nop{Additionally, we explore the limitations of using offline datasets for evaluating task completion and propose a novel, live evaluation framework on actual websites. This allows for real-time assessment and addresses the shortcomings of static simulated environments in Mind2Web. \boyuan{[add some conclusion]}

To summarize, our contributions are threefold:
\begin{itemize}
    \item We present the first quantitative analysis of GPT-4V in web navigation, establishing a performance benchmark via human evaluations.
    \item We pinpoint the challenges associated with webpage element referencing and propose three solutions underpinned by experimental findings and a comprehensive analysis of their strengths and limitations. With proper referring, our web agent based on GPT-4V achieves the best performance on Mind2Web.
    \item We introduce a novel online evaluation framework for web agents, enabling real-time performance assessments on live websites, thus overcoming the constraints of traditional simulated evaluations.
\end{itemize}
}

==> sec/2_lmm2web.tex <==
\section{LMM2Web}
\label{sec:upper_bound}
% We introduce \textbf{\ourmethod} to evaluate the suitability of GPT-4V as a generalist web agent. Concretely, given a web-related task (\eg, ``Rent a truck with the lowest rent'' in the car rental website), we check if GPT-4V possesses two essential capabilities for web navigation: (i) \textbf{Action Generation} to produce an action (\eg, ``Move the cursor over the Find Your Truck button'') to perform the current task, and (ii) \textbf{Element Referring} to identify an HTML element (\eg, ``[button] Find Your Truck'') of the current action in the webpage. Before assessing the capabilities, we first provide a brief background of web navigation.

\label{sec:background}
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/figure2.pdf}
    \caption{An example of the element referring process for a single action during completing the given task with three different methods. In this action step, the model needs to click the "Find Your Truck" button to perform a search with all required search details already filled. 
    For textual choices referring, some element candidates represented with HTML text are given, the model is required to generate the choice index of the target element. 
    For image annotation, bounding boxes and labels are added to the image. The model is required to generate the label on the top-left of the target element.  
    For element attributes referring, the model needs to predict the text and type of the target element. 
    }
\end{figure*}
\label{fig:main-figure}

We introduce our developed \textbf{\ourmethod}, a generalist web agent based on GPT-4V. 
% We explicitly ask \gptv to analyze the given task, previous actions, and screenshot, and generate an action based on its analysis and reasoning. 
Specifically, given a web-based task (\eg, ``Rent a truck with the lowest rate'' in the car rental website), we examine two essential capabilities of if GPT-4V as a web agent: (i) \textbf{Action Generation} to produce an action description\hs{a description of action sequences?} (\eg, ``Move the cursor over the `Find Your Truck' button and perform a click'' \hs{at one step}) to complete the task, and (ii) \textbf{Element Referring} to identify an HTML element (\eg, ``[button] Find Your Truck'') of the current action in the webpage. Before assessing the capabilities, we first provide a brief background and task formulation of web agents.

% \subsection{Web Navigation Background}
\subsection{Formulation}

% Given instruction $I$, a web agent should generate a sequence of executable actions $A=[\vect{a}_1, \vect{a}_2,...,\vect{a}_n]$ to accomplish the task. Each of the actions is generated given the status of the website at a time step.

% Given a browser environment $\mathcal{S}$ starting at a website and a task instruction $I$, a web agent should generate a sequence of executable actions $A=[\vect{a}_1, \vect{a}_2,...,\vect{a}_n]$ to accomplish the task. Each of the actions is generated given the status of the website at a time step.

Given a website $\mathcal{S}$ (\textit{e.g.,} \emph{``a car rental website''}) and a task $T$ (\textit{e.g.,} \emph{``Rent a truck with the lowest rate''}), the web agent should generate a sequence of executable actions $A=[\vect{a}_1, \vect{a}_2,...,\vect{a}_n]$ to complete the task. Specifically, at time step $t$, the agent should generate an action $\vect{a}_t$ based on the current environment observation ${s}_t$, the previous actions $\{\vect{a}_1, \vect{a}_2, ..., \vect{a}_{t-1}\}$, and the task $T$: 
\begin{equation}
    \vect{a}_t = \pi(s_t, T, \{\vect{a}_1, \vect{a}_2, ..., \vect{a}_{t-1}\})
\end{equation}
\label{eq:step-wise}

%Web navigation, as defined in recent works~\cite{deng2023mind2web, Yao2022WebShopTS, Zhou2023WebArenaAR, liu2018reinforcement}, is a sequential decision-making problem. In this context, web agents interact with website environments to complete tasks expressed in natural language. More specifically, the web agent is given a website (\textit{e.g.,} a car rental website), from which the web agent can derive environment observation $S$. The web agents are required to complete a task instruction expressed in natural language (\textit{e.g.,} Rent a truck with the lowest rent) on this website. The web agent needs to generate a sequence of actions $A=\{a_1, a_2, ..., a_t, ...\}$ conditioned on the task instruction $T$ and the environment observation $S$.
% Specifically, given a high-level task described in natural language, the agent's objective is to accomplish this task by generating a sequence of web navigation actions, each comprising an element of a webpage for interaction and the requisite operation to be executed on the target element. \jh{perhaps, show examples of element and operation? \eg, element:[Searchbox] Find, operation: TYPE auto repair} To complete the given task, the agent needs to be grounded in a web environment. The observation from the web environment is HTML text for text-only language models and webpage screenshots for vision-language models. \jh{should be both webpage screenshots and HTML text for VLMs?}

The environment observation $s_t$ comprises an HTML document $s_t^H$ and a screenshot image $s_t^{I}$. LLMs can only ground on the HTML document, while VLMs and LMMs can be grounded on both the HTML document and the screenshot image. The website status is updated accordingly after each action: $$s_{t+1} = \mathcal{S}(\vect{a}_t) = \{s_{t+1}^{H}, s_{t+1}^{I}\} $$ 
For simplicity, in subsequent step-wise formulations, the time step notation $t$ is omitted.

An action $\vect{a}$ corresponds to a browser event provided by the website environment. Therefore, we formulate an action as a triplet of three necessary variables for a browser event $(e, o, v)$. 
$e \in \mathcal{E}$ identifies the target webpage element to operate on, such a button (\textcolor{brown}{<button} \textcolor{red}{id}=\textcolor{blue}{2} \textcolor{red}{meta}=\textcolor{blue}{"button; tab"}\textcolor{brown}{>}Description\textcolor{brown}{</button>}). $\mathcal{E}$ represents the set of webpage elements within the environment $\mathcal{S}$. The operation $o \in \mathcal{O}$ is the action to be performed on the target element, with $\mathcal{O}$ encompassing all possible operations in $\mathcal{S}$ (\eg, \texttt{Click}, \texttt{Type}). The variable $v$ denotes the additional value needed for the operation (\eg, the date \textit{12/10/2023} for a \texttt{Type} operation).

However, agents based on LLMs or LMMs are typically unable to directly generate the three variables $(e, o, v)$ required for a browser event. Instead, they generate a textual description of the intended action $\tilde{\vect{a}}$, containing information about these variables as $(\tilde{e}, \tilde{o}, \tilde{v})$. This process is referred to as \textbf{Action Generation}. To interact with the environment, a further step is required to convert $\tilde{\vect{a}}$ into $\vect{a}$. The major challenge in this process is mapping the described element $\tilde{e}$ to an actual HTML element $\vect{e} \in \mathcal{E}$, denoted as \textbf{Element Referring}.

% However, an LLM-driven agent barely is able to generate a textual description $\tilde{\vect{a}}$ that includes information of $(\tilde{\vect{e}},\tilde{\vect{o}},\tilde{\vect{v}})$, rather than $\vect{a} =(\vect{e},\vect{o},\vect{v}) $. We denote this step as \textbf{Action Generation}. To execute and interact with the environment, we still need an extra process to convert it to $\vect{a}$. The main work here is to refer the element description $\tilde{e}$ to the actual HTML element $\vect{e} \in \mathcal{E}$. Hence we denote this step as \textbf{Element Referring}


% For the web agent, the observation $s_t$ from the environment consists of both an HTML document $s_t^H$ (\eg, \autoref{fig:teaser} and a screenshot image $S_t^{I}$ (\eg, \autoref{fig:teaser}, Right). The web environment is dependent on the type of model being used. VLMs and LMMs can use both the HTML document $H_t$ and the screenshot image $S_t^{I}$, while LLMs rely solely on the HTML document $S_t^H$. 

% Specifically, at a time step $t$, we have the status observation $S_t$ of the website in both HTML and screenshots ($S_t^\text{HTML}$ and $S_t^\text{Vision}$). The agent should generate the next action based on 

% $\vect{a}_t$ based on $(I, S_t , [\vect{a}_1, \vect{a}_2,..., \vect{a}_{t-1}])$. And the website status is updated accordingly, i.e. $S_{t+1}=\mathcal{S}(\vect{a}_t)$. We omit the notation $t$ for simplicity in further step-wise formulation.


% An action here is an executable browser event in the website environment, not only a description. Therefore, we formulate an action $\vect{a}$ as a triplet $(\vect{e},\vect{o},\vect{v})$. $\vect{e}$ is in a set of webpage elements $\mathcal{E}$ provided by the environment $\mathcal{S}$; $\vect{o}$ is from a pre-defined action space $\mathcal{O}$; $\vect{v}$ is additional values required for a specific operation. $\vect{e}$ and $\vect{o}$ can be empty for certain operations.

% However, an LLM-driven agent typically barely is able to generate a textual description $\tilde{\vect{a}}$. We denote this step as \textbf{Action Generation}. To execute and interact with the environment, we still need an extra process to convert it to its intended action. The main work here is to refer the element description $\tilde{e}$ to the actual element in $\mathcal{E}$. Hence we denote this step as \textbf{Element Referring})

% a web agent $f$ should generate an executable action $a_t$ based on the current environment $S_t$, the previous actions $\{a_1, a_2, ..., a_{t-1}\}$, and the task instruction $I$,
% \begin{equation}
%     a_{t} = f(S_t, I, \{a_1, a_2, ..., a_{t-1}\})
% \end{equation}
% \label{eq:step-wise}

%The webpage element $e_t \in E$, identified by a node ID (\textit{e.g.,} <input id=11 button find your truck />), is a specific element on the webpage. The set of all such elements on the webpage defines the space of webpage element $E$, introducing significant complexity to action generation. \jh{perhaps provide some numbers to show how complex it is?}
%The operation type $o_t \in O$ refers to the kind of operation on the webpage (\textit{e.g.,} CLICK or TYPE). The set $O$ encompasses all possible operations on the webpage. Finally, the operation value $v_t$ is the necessary input for the operation (\textit{e.g.,} the date for picking up the rented car in a TYPE operation).

% For web agent, the environment $S_t$, consists of a HTML document $H_t$ (\eg, \autoref{fig:teaser}, Left) and a webpage $I_t$ (\eg, \autoref{fig:teaser}, Right). This web environment is dependent of the type of model being used. For instance, Vision-Language Models (VLMs) and Language Model Multimodal (LMM) can use both the HTML document $H_t$ and the screenshot $I_t$, while Large Language Models (LLMs) rely solely on the HTML document $H_t$. After this action, the environment observation will be updated to $S_{t+1} = \{S_{t+1}^{HTML}, S_{t+1}^{Screenshot}\}$.

% Besides, the action $a_{t} = (e_t, o_t, v_t)$ is a triplet including a HTML element $e_t$ (\eg, \textit{<div backend\_node\_id="67170">When do you want to pick up your truck?</div>}) and an operation $o_t$ along with its value $v_t$ (\eg, \textit{TYPE} and \textit{"12/10/2023"}). To execute an operation at time step $t$, the agent should correctly predict all the three parts.

%At time step $t$, the web agent needs to generate the next step action on the website conditioned on the current environment observation, the history of past actions, and the task instruction. The environment observation at time $t$, denoted as $s_t$, includes both the webpage's HTML document $s_t^{HTML}$(\textit{e.g.,} as illustrated on the left side of Figure~\ref{fig:teaser}) and a screenshot image $s_t^{Screenshot}$ (\textit{e.g.,} as shown on the right side of Figure~\ref{fig:teaser}). The action history up to time $t$ is represented as $H_t = A_{1:t-1}={a_1, ..., a_{t-1}}$. The action at time $t$ is formulated as:
%\begin{equation}
%    a_{t} = \Psi (T, s_t, \{a_1, a_2, ..., a_{t-1}\})
%\end{equation}
%\label{eq:step-wise}
%In formula~\ref{eq:step-wise}, $\Psi$ represents the model for inference. For Vision-Language Models (VLM) and Language Model Multimodal (LMM), the observation $s_t$ is the HTML document $s_t^{HTML}$. For Large Language Models (LLM), the observation is the visual data $s_t^{Screenshot}$. After this action, the environment observation will be updated to $s_{t+1} = \{s_{t+1}^{HTML}, s_{t+1}^{Screenshot}\}$.

%The action $a_{t} = (e_t, o_t, v_t)$ is a triple comprising a webpage element $e_t$, an operation type $o_t$, and an operation value $v_t$. The webpage element $e_t \in E$, identified by a node ID (\textit{e.g.,} <input id=11 button find your truck />), is a specific element on the webpage. The set of all such elements on the webpage defines the space of webpage element $E$, introducing significant complexity to action generation. The operation type $o_t \in O$ refers to the kind of operation on the webpage (\textit{e.g.,} CLICK or TYPE). The set $O$ encompasses all possible operations on the webpage. Finally, the operation value $v_t$ is the necessary input for the operation (\textit{e.g.,} the date for picking up the rented car in a TYPE operation).

% At each step of decision-making, the agent is tasked with generating an action that can be converted into a browser event. The action generation is conditioned on the task description, the history of actions that have been taken, and the observation from the environment. Each web navigation action encompasses: (1) \textbf{Webpage Element}, which must be as precise as a specific node ID on the webpage to ensure accurate element localization. (2) \textbf{Operation Type}, the kind of action operation in predefined action space, like "CLICK". (3) \textbf{Operation Value}, indicating the necessary input for the web navigation action. 

% For example, in Figure~\ref{fig:teaser}, the agent's task is "Rent a Truck" within the web environment of Truck Rental website. In vision-language models, such as GPT-4V, the observation comprises a screenshot from the truck rental website's homepage. For text-only models like GPT4, the observation is limited to the HTML text used to rendering the screenshot. As illustrated in Figure~\ref{fig:teaser}, a relatively small portion of the webpage screenshot necessitates a substantial volume of HTML text for its generation.

% Webpage environment usually contains thousands of elements, leading to an action space with high complexity and a context exceeding the max token length of language model. Two-stage strategy is taken to deal with this challenge by firstly selecting candidate elements and action prediction based on the selected context.\jh{perhaps elaborate it more about how it selects the candidate elements?} \citet{deng2023mind2web} utilized a cross-encoder for element ranking and \cite{Zhou2023WebArenaAR} 

% \textbf{Action Generation} During each step of action generation, GPT4-Vision initially produces a description for the subsequent action. This description encompasses both a high-level strategy and detailed, low-level steps. Mostly, these steps will be preceded by intermediate thoughts. The quality of generation at this stage represents the upper limit of the model's capability in web navigation tasks. In Section~\ref{sec:upper_bound}, we implement human annotation to manually determine whether the generated intermediate thoughts and action descriptions adequately capture the essence of the intended target element and action.


% \boyu{[Boyu: 

% I still prefer this version to emphasize the difference between $\tilde{\vect{a}}$ and $\vect{a}$, and clearly formulate most of the things in this part (2.1 Formulation)]:

% Given a browser environment $\mathcal{S}$ starting at a website and a task Intent $I$, a web agent should generate a sequence of executable actions $A=[\vect{a}_1, \vect{a}_2,...,\vect{a}_n]$ to accomplish the task. Each of the actions is generated given the status of the website at a time step.

% Specifically, at a time step $t$, we have the status observation $s_t$ of the website in both HTML and screenshots ($s_t^H$ and $s_t^V$). The agent needs to decide the next action $\vect{a}_t$ based on $(I, s_t , [\vect{a}_1, \vect{a}_2,..., \vect{a}_{t-1}])$. And the website status is updated accordingly, i.e. $S_{t+1}=\mathcal{S}(\vect{a}_t)$. We omit the notation $t$ for simplicity in further step-wise formulation.

% An action here is an executable browser event in the website environment, not only a description. Therefore, we formulate an action $\vect{a}$ as a triplet $(\vect{e},\vect{o},\vect{v})$. $\vect{e}$ is from a set of webpage elements $\mathcal{E}$ provided by the environment $\mathcal{S}$; $\vect{o}$ is from a pre-defined action space $\mathcal{O}=\{\vect{o}_1, \vect{o}_2, ... \}$ (For example, "Click", "Type", "Select", "HOVER", "Scroll"); $\vect{v}$ is additional values required for the operation. $\vect{e}$ and $\vect{o}$ can be empty for certain operations.

% However, an LLM-driven agent barely is able to generate a textual description $\tilde{\vect{a}}$ that includes information of $(\tilde{\vect{e}},\tilde{\vect{o}},\tilde{\vect{v}})$, rather than $\vect{a} =(\vect{e},\vect{o},\vect{v}) $. We denote this step as \textbf{Action Generation}. To execute and interact with the environment, we still need an extra process to convert it to $\vect{a}$. The main work here is to refer the element description $\tilde{e}$ to the actual HTML element $\vect{e} \in \mathcal{E}$. Hence we denote this step as \textbf{Element Referring}}


% a web agent $f$ should generate an executable action $a_t$ based on the current environment $S_t$, the previous actions $\{a_1, a_2, ..., a_{t-1}\}$, and the task instruction $I$,
% \begin{equation}
%     a_{t} = f(S_t, I, \{a_1, a_2, ..., a_{t-1}\})
% \end{equation}
% \label{eq:step-wise}

%The webpage element $e_t \in E$, identified by a node ID (\textit{e.g.,} <input id=11 button find your truck />), is a specific element on the webpage. The set of all such elements on the webpage defines the space of webpage element $E$, introducing significant complexity to action generation. \jh{perhaps provide some numbers to show how complex it is?}
%The operation type $o_t \in O$ refers to the kind of operation on the webpage (\textit{e.g.,} CLICK or TYPE). The set $O$ encompasses all possible operations on the webpage. Finally, the operation value $v_t$ is the necessary input for the operation (\textit{e.g.,} the date for picking up the rented car in a TYPE operation).

% For web agent, the environment $S_t$, consists of a HTML document $H_t$ (\eg, \autoref{fig:teaser}, Left) and a webpage $I_t$ (\eg, \autoref{fig:teaser}, Right). This web environment is dependent of the type of model being used. For instance, Vision-Language Models (VLMs) and Language Model Multimodal (LMM) can use both the HTML document $H_t$ and the screenshot $I_t$, while Large Language Models (LLMs) rely solely on the HTML document $H_t$. After this action, the environment observation will be updated to $S_{t+1} = \{S_{t+1}^{HTML}, S_{t+1}^{Screenshot}\}$.

% Besides, the action $a_{t} = (e_t, o_t, v_t)$ is a triplet including a HTML element $e_t$ (\eg, \textit{<div backend\_node\_id="67170">When do you want to pick up your truck?</div>}) and an operation $o_t$ along with its value $v_t$ (\eg, \textit{TYPE} and \textit{"12/10/2023"}). To execute an operation at time step $t$, the agent should correctly predict all the three parts.

%At time step $t$, the web agent needs to generate the next step action on the website conditioned on the current environment observation, the history of past actions, and the task instruction. The environment observation at time $t$, denoted as $s_t$, includes both the webpage's HTML document $s_t^{HTML}$(\textit{e.g.,} as illustrated on the left side of Figure~\ref{fig:teaser}) and a screenshot image $s_t^{Screenshot}$ (\textit{e.g.,} as shown on the right side of Figure~\ref{fig:teaser}). The action history up to time $t$ is represented as $H_t = A_{1:t-1}={a_1, ..., a_{t-1}}$. The action at time $t$ is formulated as:
%\begin{equation}
%    a_{t} = \Psi (T, s_t, \{a_1, a_2, ..., a_{t-1}\})
%\end{equation}
%\label{eq:step-wise}
%In formula~\ref{eq:step-wise}, $\Psi$ represents the model for inference. For Vision-Language Models (VLM) and Language Model Multimodal (LMM), the observation $s_t$ is the HTML document $s_t^{HTML}$. For Large Language Models (LLM), the observation is the visual data $s_t^{Screenshot}$. After this action, the environment observation will be updated to $s_{t+1} = \{s_{t+1}^{HTML}, s_{t+1}^{Screenshot}\}$.

%The action $a_{t} = (e_t, o_t, v_t)$ is a triple comprising a webpage element $e_t$, an operation type $o_t$, and an operation value $v_t$. The webpage element $e_t \in E$, identified by a node ID (\textit{e.g.,} <input id=11 button find your truck />), is a specific element on the webpage. The set of all such elements on the webpage defines the space of webpage element $E$, introducing significant complexity to action generation. The operation type $o_t \in O$ refers to the kind of operation on the webpage (\textit{e.g.,} CLICK or TYPE). The set $O$ encompasses all possible operations on the webpage. Finally, the operation value $v_t$ is the necessary input for the operation (\textit{e.g.,} the date for picking up the rented car in a TYPE operation).

% At each step of decision-making, the agent is tasked with generating an action that can be converted into a browser event. The action generation is conditioned on the task description, the history of actions that have been taken, and the observation from the environment. Each web navigation action encompasses: (1) \textbf{Webpage Element}, which must be as precise as a specific node ID on the webpage to ensure accurate element localization. (2) \textbf{Operation Type}, the kind of action operation in predefined action space, like "CLICK". (3) \textbf{Operation Value}, indicating the necessary input for the web navigation action. 

% For example, in Figure~\ref{fig:teaser}, the agent's task is "Rent a Truck" within the web environment of Truck Rental website. In vision-language models, such as GPT-4V, the observation comprises a screenshot from the truck rental website's homepage. For text-only models like GPT4, the observation is limited to the HTML text used to rendering the screenshot. As illustrated in Figure~\ref{fig:teaser}, a relatively small portion of the webpage screenshot necessitates a substantial volume of HTML text for its generation.

% Webpage environment usually contains thousands of elements, leading to an action space with high complexity and a context exceeding the max token length of language model. Two-stage strategy is taken to deal with this challenge by firstly selecting candidate elements and action prediction based on the selected context.\jh{perhaps elaborate it more about how it selects the candidate elements?} \citet{deng2023mind2web} utilized a cross-encoder for element ranking and \cite{Zhou2023WebArenaAR} 

% \textbf{Action Generation} During each step of action generation, GPT4-Vision initially produces a description for the subsequent action. This description encompasses both a high-level strategy and detailed, low-level steps. Mostly, these steps will be preceded by intermediate thoughts. The quality of generation at this stage represents the upper limit of the model's capability in web navigation tasks. In Section~\ref{sec:upper_bound}, we implement human annotation to manually determine whether the generated intermediate thoughts and action descriptions adequately capture the essence of the intended target element and action.
% }

\subsection{Action Generation}
\label{sec:action-generation}

% \gptv\ cannot directly generate a program for web agent actions. Instead, it tends to generate textual descriptions of target actions, labeled as $a_t^{'}$ (\textit{e.g.,} the description about clicking "Find Your Truck" Button in Figure~\ref{fig:main-figure}) 

\gptv\ is explicitly instructed to imitate human web browsing and analyze the task, webpage, and previous actions, as shown in Table~\ref{tab:task_generation_prompt}. Finally, it is asked to generate an action description $\tilde{a}$ based on its analysis and reasoning, which should encapsulate necessary details to help identify the intended action $\vect{a}$. We take the screenshot image $s^I$ as the visual context without utilizing the HTML document $s^H$ for action generation.

An ideal action description should thoroughly encapsulate all necessary details to precisely identify the intended action $a$. Specifically, each variable $(e, o, v)$ in the action triplet should be able to be derived from the corresponding description $(\tilde{e}, \tilde{o}, \tilde{v})$. 

Given that the model's performance is contingent upon both action generation and element referring, evaluating the performance of action generation poses a significant challenge. To assess the action generation performance, we need an oracle method to convert action description $\tilde{a}$ to action triple $a$ that can ensure as long as  the description includes necessary details about each action triple, it should be converted correctly, which ensures no mistake is caused during the conversion process.  We approximate the oracle method by asking human annotators to identify the model's intended actions.

% We approximate the oracle method by asking human annotators to judge whether the action descriptions $\tilde{a}_t$ possess sufficient information to derive the target action. Each action is labeled by two annotators who determine if the description adequately identifies the target element $e_t$, operation type $o_t$, and assigns a label to the target value $v_t$. This performance scores with the oracle conversion method is considered as the performance upper limit of \gptv\ as web agent.

% \boyu{Temporarily ignoring element referring, the model's ability to accurately identify the correct action reflects its potential. Hence we propose employing an oracle method to map $\tilde{\vect{a}}$ to action $\vect{a}$, as if an oracle could comprehensively interpret the model's intentions. We approximate the oracle method by asking human annotators to identify the model's intended actions.
% }

% We ask two annotators to score each example and use the average score as the final result. Annotators need to make sure as long as there is a description of the target action in the generated action, the described element must be referred to correctly. Human annotators need to determine whether the generated action descriptions contain adequate and valid information to derive the target webpage element, operation, and operational values.  We ask two annotators to score each example and use the average score as the final result.

% To get a better intuition about GPT-4V's performance cap, we need assume there exist a golden truth referring method that can always convert the generated action description into the corresponding action and refer to a specific element. We involve human annotators to serve as the ground truth referring method. This evaluation serves as a metric for the model’s potential in web-based tasks.

\subsection{Element Referring}
\label{sec:referring}
Despite the capability of \gptv in identifying and describing the next action to complete the given task, it is still a challenge to convert the action description $\tilde{\vect{a}}$ into a concrete action $\vect{a}$. Deriving operation type $\vect{o}$ and value $\vect{v}$ from the action description $\tilde{a}$ can be well solved through string parsing. However, identifying the target element $\vect{e}$ from generated $\tilde{\vect{e}}$ remains challenging.

To address this issue, we explore three approaches using different media to bridge the referring gap: Element Attributes, Textual Choices, and Image Annotation, as depicted in Figure~\ref{fig:main-figure}.


\paragraph{Element Attributes.}
\label{referring:exp3}
% \jh{Perhaps, the order of approaches in the text should matches the order in Figure2. (\eg, Textual Choices --> Image Annotation --> Element Attributes)}
This approach involves prompting the model to generate specific attributes of the target element, thereby providing precise information to match the description to the target HTML element. Utilizing these attributes, a heuristic search (as described in \ref{sec:exp_3}) is performed within the webpage's HTML elements to locate the element. 

Specifically, we prompt the model (as demonstrated in Table~\ref{tab:exp3}) to not only describe the element $\vect{e}$, but also specify the target element's type and the textual content in $\tilde{\vect{e}}$. For example, as illustrated in Figure~\ref{fig:main-figure}, the model would generate element text as "Find Your Truck" and identify its type as a "BUTTON." 

Following this, a heuristic search is performed across the DOM elements, using the element text and type to locate matching elements. In cases where a singular match is found, it is automatically selected. Conversely, when multiple matches arise, the model is further prompted to select the final selection.

\paragraph{Textual Choices}
\label{referring:exp4}

The above approach demands precise and sufficient attribute descriptions from \gptv\ and accurate matching by the heuristic search, which might be too demanding. For instance, many elements have no textual content or have textual information in a nearby element.

Alternatively, we can provide the model with textual representations of elements as choices to facilitate referring, which has already been proven effective in MindAct~\cite{deng2023mind2web}. Specifically, we adopted the MindAct approach in Mind2Web\cite{deng2023mind2web}. It utilizes a ranker model to select top-$k$ candidate elements $(e_1,e_2, ..., e_k)$ with a pretrained cross-encoder. Each candidate element is then represented as a choice in a multi-choice question with its HTML text indexed with a choice $c_1$, as illustrated in Fig.~\ref{fig:main-figure}.

% Specifically, we adopted the element ranker used in ~\citet{deng2023mind2web} to pick top-k candidate elements with a pretrained cross-encoder. Each candidate element is represented with its HTML text $e_i^{'}$ and a choice label $c_i$ in front to index elements.  For example, in Figure~\ref{fig:main-figure}, the element is represented as \boyu{[Boyu: It seems that you mentioned the wrong choice here?]} \textit{C: <div backend\_node\_id="67170">When do you want to pick up your truck?</div>}.
% \begin{equation}
%     E = \{
% (c_{0}, e_0^{'}), 
% (c_{1}, e_1^{'}), 
% ..., 
% (c_{k}, e_k^{'}),
% \}
% \end{equation}
% \label{eq:refer-text-choice}

After generating action description $\tilde{\vect{a}}$, the model is further asked a multi-choice question to compare its intended action $\vect{a}$ against choices in $C=\{(c_1,e_1),(c_2,e_2), ..., (c_k,e_k),(c_{k+1},\phi)\}$. Here $\phi$ represents none of the elements is the target element. The model is instructed to predict the choice label $c$ to identify the target element $e$. 

\paragraph{Image Annotation}
\label{referring:exp2}

Referring with textual representation heavily depends on the model's ability to link textual representations with corresponding image elements. However, textual representations alone are sometimes insufficient to distinguish elements that share similar descriptions, as illustrated in Fig.~\ref{fig:ambiguous-text-choice-1} and Fig.~\ref{fig:ambiguous-text-choice-2}. To address this challenge, we propose to overlap visual marks on top of the screenshot image for more precise element identification.

% \citet{Yang2023SetofMarkPU, Yan2023GPT4VIW} have shown that image annotations, including bounding boxes, masks, and text labels, significantly aid in visual question answering and object detection, and mobile UI understanding tasks. Nonetheless, the effectiveness of such annotations in complex web navigation scenarios has not been thoroughly explored.

% \boyuan{Define image annotation}
% We will provide each action generation step with some candidate choices selected by the ranking model. 
% $$E_t^{'} = \{e_t^{0'}, e_t^{0'}, ..., e_t^{k'}\}$$

Specifically, we overlay the bounding box for element $e$ and alphabet labels for $c$ on top-left of each bounding box~\footnote{We leveraged Supervision library for image annotation: \url{https://supervision.roboflow.com/}} in choices $C=\{(c_1,e_1),(c_2,e_2), ..., (c_k,e_k),(c_{k+1},\phi)\}$. The model is expected to generate the alphabetical label corresponding to the target element.

% \paragraph{Human Referring}
% \label{referring:human}
% To get a better intuition about GPT-4V's performance cap, we need assume there exist a golden truth referring method that can always convert the generated action description into the corresponding action and refer to a specific element. We involve human annotators to serve as the ground truth referring method. This evaluation serves as a metric for the model’s potential in web-based tasks.

% We ask two annotators to score each example and use the average score as the final result. Annotators need to make sure as long as there is description about the target action in the generated action, the described element must be referred correctly. Human annotators need to determine whether the generated action descriptions contain adequate and valid information to derive the target webpage element, operation, and operational values.  We ask two annotators to score each example and use the average score as the final result.

% \paragraph{Human Referring}
% \label{referring:human}
% To get a better intuition about GPT-4V's performance cap, we need assume there exist a golden truth referring method that can always convert the generated action description into the corresponding action and refer to a specific element. We involve human annotators to serve as the ground truth referring method. This evaluation serves as a metric for the model’s potential in web-based tasks.

% We ask two annotators to score each example and use the average score as the final result. Annotators need to make sure as long as there is description about the target action in the generated action, the described element must be referred correctly. Human annotators need to determine whether the generated action descriptions contain adequate and valid information to derive the target webpage element, operation, and operational values.  We ask two annotators to score each example and use the average score as the final result.

==> sec/4_results.tex <==
\section{Results and Analysis}


\subsection{Offline Evaluation Results}


\noindent \textbf{\gptv\ can be a Generalist Web Agent with Oracle Action Grounding.}
Given an effective action grounding method, \gptv\ has the potential to serve as a generalist web agent. Specifically, as described in \autoref{sec:referring}, we provide \gptv\ with an oracle action grounding method (\lmmweb\textsubscript{Oracle}) through human annotation, the model achieves a step success rate of \num{65.7}\%, \num{70.0}\%, and \num{62.1}\% across three test splits, respectively. As shown in \autoref{tab:main}, this method substantially outperforms other models under all metrics across three test splits. 
Specifically, it achieves a \num{11.9}\% step success rate improvement over the second-best method in the Cross Task setting. 
The performance advantage is more pronounced under the Cross-Website and Cross-Domain settings, where it leads by 28.3\% and 21.2\% step success rates, demonstrating its generality compared with supervised fine-tuning.
This observation is further corroborated with in the online evaluation (\autoref{tab:online_evaluation}).


\noindent \textbf{Element Grounding Method Comparison.}
However, there is a noticeable gap between oracle grounding and all the three proposed grounding methods. 
This demonstrates that grounding, especially element grounding, is a major bottleneck. 
Element grounding via textual choice (\lmmweb\textsubscript{Choice}) demonstrates the best performance under all metrics across all settings,  comparable to supervised fine-tuning and showing a substantial improvement over text-only LLMs.

Grounding via image annotation (\lmmweb\textsubscript{Annotation}) offers an intuitive approach and shows promising results in recent work that focuses on object- or scene-centric images~\cite{Yang2023SetofMarkPU}. 
% It aims to clarify the ambiguities inherent in text-only HTML representations by incorporating image-based annotations. 
However, we find that on complex images with rich semantic and spatial relationships like webpage screenshots, severe hallucination is observed from GPT-4V. 
Specifically, it often fails to correctly map its generated element description (which is often correct according to oracle grounding) to the right bounding box and index label in the image, leading to a low element accuracy.
% Specifically, as it achieves a very low Element Accuracy, even though its Operation F1 scores are comparable to \lmmweb\textsubscript{Choice}, the Step Success Rate is still low. 
This limitation primarily arises from \gptv's weakness in understanding image details and relative spatial location, a topic that we will further delve into in \autoref{sec:problems}.

Grounding via element attributes (\lmmweb\textsubscript{Attribute}) also demonstrates inferior performance. This method's effectiveness is primarily limited by its heuristic-based element localization strategy, which depends on textual and locality characteristics. This becomes problematic as not all webpage elements contain text, and sometimes the relevant text is associated with a nearby but distinct element.
% \hs{(see an error example in XX)}.



\noindent \textbf{LMMs vs. LLMs.}
The \lmmweb\textsubscript{Choices} model demonstrates a substantial performance advantage over the text-only GPT-4 under all three metrics across all three test splits. Specifically, it outperforms GPT-4 in step success rate of 8.9\%, 14.7\%, and 11.2\% on three settings, respectively.
Interestingly, fine-tuned BLIP-2-T5 does not show a noticeable gain over FLAN-T5, despite having additional visual input. 
Several factors may contribute to this. First, the CLIP model used as the image encoder may not be sufficiently adept at image details, as explored by \citet{shen2021much}. This limitation is particularly relevant for our web navigation task, which demands a high level of image detail comprehension. Second, BLIP-2-T5 utilizes an off-the-shelf CLIP model that may not be optimal for webpage screenshots.
Finally, although the screenshots in the test splits are error-free, some of the examples in the training set might contain issues such as rendering failures or inaccuracies in the timing of screenshot capture by annotators. 


\noindent \textbf{SFT vs. ICL.}
We compare SFT and ICL methods to offer insights for developing web agents in different scenarios. ICL (with \ourmethod) demonstrates consistent and robust performance across three test splits. 
ICL is particularly advantageous in scenarios lacking annotations or requiring strong generalization capabilities for new domains and websites. As grounding methods improve towards oracle grounding, ICL is poised to show even stronger performance.
On the other hand, SFT methods show better generalization across tasks on websites already seen during training. 
Considering the high cost of data annotation for web agents and the billions of websites on the Internet, ICL offers a more compelling solution for generalist web agents.
However, if one only needs to develop a strong web agent for a certain website, SFT is still a competitive solution. 
% The fine-tuned FLAN-T5 model shows the best performance under the Cross-Task setting and outperforms \lmmweb\textsubscript{Choices} by \num{11.9}\%. 


\subsection{Online Evaluation Results}
%In online evaluation, we allow the web agent to keep running, and the human annotator was tasked to determine whether each task was successfully completed. 
In online evaluation, we pair a web agent with a human annotator, where the human was tasked to monitor agent actions that may change real-world states and determine whether each task was successfully completed. For comparative analysis, we include success rates from offline evaluation, denoted as Offline\textsubscript{0} (allowing zero wrong action) and Offline\textsubscript{1} (allowing one wrong action).

\begin{table}[t]
\centering
\small
\tabcolsep 3.5pt
\renewcommand\arraystretch{1.0}
\begin{tabular}{lccc}
\toprule
% \multirow{2}{*}{} &
% \multicolumn{3}{c}{Cross-Task} &
% \multicolumn{3}{c}{Cross-Website} &
% \multicolumn{3}{c}{Cross-Domain} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
& Offline\textsubscript{0}& Offline\textsubscript{1} & Online \\
\midrule
FLAN-T5-XL&\num{2}&\num{20}& \num{18}   \\
GPT-4 &\num{2}&\num{18}&\num{20}   \\
\lmmweb\textsubscript{Choice} &\num{8}&\num{22}& \num{26}\\
\lmmweb\textsubscript{Oracle} &\num{18}&\num{58}&\num{50}\\

\bottomrule
\end{tabular}
\vspace{-5pt}
%\captionsetup{width=0.95\textwidth} 
\caption{Whole task success rate (\%) under both offline and online evaluation. Offline\textsubscript{0} and Offline\textsubscript{1} refer to no tolerance for error at any step and allowing for error at one step, respectively. 
% \hs{can we include the message here that 'Under online evaluation, XX gets all tasks successfully completed while YY gets over half the tasks'? oh, i somehow thought 50 means 50 tasks...}
}
%Offline\textsubscript{0} and Offline\textsubscript{0} refer to tolerance for error at zero or one action step.  \hs{}}
\label{tab:online_evaluation}
\end{table}


Table~\ref{tab:online_evaluation} shows that the whole task success rate in online evaluation substantially exceeds that of offline evaluation (Offline\textsubscript{0}). This finding suggests that the whole task success rate is likely underestimated in the offline evaluation due to the variability in actions and plans.
In other words, there may be multiple viable plans for a task, but the reference plan in offline evaluation only captures one of them. 

Across all three settings, \lmmweb\textsubscript{Choice} outperforms both GPT-4 and FLAN-T5-XL. Using oracle grounding further improves the performance substantially, reaching a remarkable whole task success rate of \num{50}\%.
Although GPT-4 shows much worse performance than FLAN-T5-XL in step success rate under offline evaluation (\autoref{tab:main}), they exhibit similar success rates in online evaluation. These results further confirm the potential of large models for generalist web agents compared with fine-tuned small models. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/sr_by_action_length_difficulty.pdf}
    \caption{Whole task success rate across task difficulty levels. We categorize tasks based on the number of actions to complete, i.e., Easy: \num{2}-\num{4}, Medium: \num{5}-\num{7}, and Hard: \num{8}-\num{12}, with \num{26}, \num{15}, and \num{9} tasks in each group, respectively.}
    \label{fig:sr_difficulty}
\end{figure}

\noindent\textbf{Online Success Rate by Task Difficulty.}
We investigate the performance of web agents on tasks across different difficulty levels. We estimate the task difficulty based on the number of actions taken by annotators during action trace annotation. %We categorize tasks into three levels based on the number of actions: [2, 3, 4], [5, 6, 7], and [8, 9, 10, 11, 12], with 26, 15, and 9 tasks in each group, respectively. 
As shown in \autoref{fig:sr_difficulty}, the whole task success rate is negatively correlated with the number of actions---it decreases as the number of actions increases across all four methods. \lmmweb\textsubscript{Oracle} consistently outperforms other methods across all difficulty levels. 
Interestingly, the gap between \lmmweb\textsubscript{Oracle} and \lmmweb\textsubscript{Choice} enlarges on longer-horizon tasks.
This is understandable because grounding errors cascade to later steps; nonetheless, it further shows the challenge of grounding for GPT-4V and the need for better grounding methods.


\subsection{Quantitative Analysis}

% \noindent\textbf{OSS v.s. API.} 
% Open-sourced models have emerged as important competitors of APIs, like GPT4V and Gemini. 
% OSS models show advantages in offline evaluation with a large performance margin over both GPT4V and Gemini but still lag behind the performance of GPT4V with the Oracle grounding method. 
% However, they may not generalize well enough to the online evaluation setting, considering FLAN-T5 lost its advantages over GPT4 on online evaluation. OSS has the advantage of flexibility by fine-tuning the model to allow grounding with pixel-level location, as shown in CogAgent performance. 


\noindent\textbf{Error Analysis in Grounding via Image Annotation.} 
Set-of-mark prompting~\cite{Yang2023SetofMarkPU} uses a similar method as grounding via image annotation and has been shown effective on object- or scene-centric images~\cite{Lin2014MicrosoftCC, Plummer2015Flickr30kEC, Zhou2017ScenePT}. However, this grounding method is suboptimal on webpage screenshot images that are complex and contain rich semantic and spatial relationships.

To analyze the reasons behind the failures, we randomly sample \num{100} predicted actions and observe the major types of errors as: (1) Wrong action generation; (2) Making up bounding box \& label; (3) Failure to link bounding boxes with the correct labels. Illustrative examples are included in \autoref{sec:hallucination-examples}.

Our analysis reveals that \num{53}\% of the errors originate from wrong action generation wherein the model fail to predict the target element within the action description.
This error rate is \num{27}\% higher than images without annotation, which exhibits a \num{26}\% error rate because image annotation often obscures critical content within webpages. 
Overlaying image annotations on webpages without obscuring important content poses a significant challenge. This is primarily due to the dense layout of webpages, which often feature small elements designed for precise cursor interactions. In contrast, the arrangement of objects in mobile UIs and natural scenes tend to be sparser.

Then \num{21}\% of the errors can be attributed to \gptv's tendency of visual illusion~\cite{Guan2023HallusionBenchAA}, where the model misinterprets and fabricates content over the image. Specifically, the target element described in action generation does not have a bounding box or a label on the bottom-left, where the model is supposed to generate "None". However, the model falsely assumes the presence of a bounding box and makes up a label as the answer. Another \num{18}\% of errors are caused by \gptv's limitation in recognizing the relative position within an image. Specifically, the model is capable of identifying both the target element within the bounding box and the labels. However, it struggles to link the bounding box with its corresponding label.

% \noindent\textbf{Pixel-level Grounding Analysis.}
% In parallel with the three grounding methods we studied in SeeAct, the pixel-level grounding by generating coordinates on the image is popular for OSS models. We conduct human annotation on the results of pixel-level grounding on CogAgent to check the results. \boyuan{Add Analysis result}



\subsection{Qualitative Study}

\noindent\textbf{Powerful Web Action Planner.} 
\gptv\ exhibits promising capabilities, ranging from speculative planning, webpage content reasoning, and error correction to surpassing the limitations of superficial textual similarity matching inherent in fine-tuned, text-only models.
\gptv\ exhibits capability in speculative planning involving a series of interconnected low-level actions. As illustrated in \autoref{appendix_case_planning}, besides generating the immediate next step action, the model also anticipates a sequence of subsequent actions in the future to complete the given task. 
% model not only suggests immediate actions on the homepage but also anticipates subsequent steps in the future. It devises comprehensive plans that address every facet of the task, demonstrating foresight even in the initial stages.

\noindent\textbf{Error Correction Awareness.} 
\gptv\ also exhibits the awareness of error correction in the previous actions. In the example in \autoref{appendix_case_path}, \gptv\ is capable of discovering the mobile phone number is invalid due to wrong format and generate the description about the action to correct this error. This highlights the model's potential for adaptation in online settings, where actions may not always follow pre-defined, ideal paths as in offline evaluations. This error-correction capability paves the way for adding robustness and reasonable dynamic planning.

% \gptv\ is capable of attending to both history and the current webpage environment. \autoref{fig:case-understanding} shows a challenging query where two crucial pieces of information had not been recorded in the history, namely the filled "Drop-off Date" and the clicked "No" button. However, \gptv\ realized these two pieces of evidence from close examination and made the right decision. 


% \noindent\textbf{Powerful Web Action Planner}

% -- gpt4v is powerful at a lot of things: from the lower level image understanding, reasoning on the webpage, and even longer range decent planning actions that are far beyond (textual similarity matching) what fine-tuned models and text-only generalist models are capable of. \\
% -- Shows some examples to explain in detail. 

% In \ourmethod , we explicitly instruct the model analyze the webpage and previous history to make it understand the environment and history. Fig.~\ref{fig:case-understanding} shows its impressive ability in doing this. This query is challenging because two crucial information had not been recorded in the history, namely the filled "Drop-off Date" and the clicked "No" button. However, \gptv\ found this two evidences from its close examination, and hence made the right decision. 
% During action generation, \gptv could not only determine the correct current step, but also the subsequent actions. Fig. \boyu{[Boyu: Find a case GPT4V directly chose several element and give corresponding actions. There are a lot]} shows that \gptv\ directly gives a serious actions in the webpage, even we had emphasize it only should generate only the next action. And what's even surprising is that it could even foresee the approximate next steps in later webpages. In the case of Fig.~\ref{fig:planning}, it suggested not only the current step in the homepage, but also the later steps in later sections. And it generated the whole plan to satisfy every aspect of the task, even if it is only a start stage.

% \boyu{Boyu: The awareness of error correction can be either in Powerful planner or Action/path variation.

% Awareness of Error correction

% Fig. \boyu{\ref{fig:case-error-correction}} is a "wrong" answer in offline, but it reflects that the model has an awareness of correcting the errors caused by previous steps.

% It's more often in online, and is more crucial in online. 

% A key difference between offline and online is that, the previous actions are not golden annotated actions. Here it does not only mean simple cases that involves interchangeable steps, but also mean the previous actions may have caused fatal errors or even totally wrong, which lead to a webpage that is far away from the goal.
% Hence online testing really requires the model to have an awareness of correcting its errors and move it to the correct direction.
% }

\noindent\textbf{Advantages of Knowledge.}
\gptv\ demonstrates substantial advantages in tasks that requires certain knowledge over fine-tuned models at a smaller scale. As shown in \autoref{appendix_case_knowledge}, \gptv\ is able to identify the IATA code of the airport in Los Cabos as SJD. In contrast, models are typically weaker at knowledge intensive tasks and also likely to lose knowledge during the fine-tuning process due to catastrophic forgetting. 

% Despite this, fine-tuned models exhibit promising performance in generating actions for low-level tasks. This opens up an intriguing possibility: integrating the strengths of both generalist and fine-tuned models. By employing generalist models like \gptv\ for breaking down complex tasks into manageable components and utilizing supervised fine-tuned models for executing specific low-level actions, a more robust and effective approach to task execution can be achieved. Such a hybrid system could potentially combine the depth of specialized knowledge with the precision of task-specific actions.


% \noindent\textbf{Variability of Action and Path Variation}
% One of the intrinsic aspects of task completion is the variability of actions, which is critical yet beyond the capability of offline evaluation. For instance, filling out forms can vary significantly, as referenced in the AA form example. Additionally, some web pages feature multiple links leading to the same destination, all of which should be considered valid. 

% In online testing, this variability extends to the level of webpage navigation, not just actions within a single page, as illustrated in the simple path variation example in \autoref{fig:path}. A more intricate and frequent scenario involves the agent either forgetting or failing to execute a required action yet managing to rectify this in subsequent steps. In addition, there are instances where the agent may not immediately know the correct action, leading to exploratory or incorrect steps. These situations highlight that the agent's path can significantly diverge from predefined action paths. However, as shown in previous examples (e.g., Figure 6 or other online case studies), the model is able to find its way back to the correct trajectory. 

% While offline evaluations can provide some measure of an agent's capabilities, embracing an online environment is preferable. This approach allows for varied paths and acknowledges the agent's ``explorations'' and mistakes as part of the learning and adaptation process on a website.


% A more complex and common phenomenon is that, the agent may forget or fail to execute an action that it should do, but it may fix it in later steps. And also it may have no idea how to do it right now, so it does some kind of exploration (false step). To conclude, the path can be far deviated from the annotated action paths. And both in the two cases, the model may generally go back to the correct route. \boyu{ref the previous Fig.6 or other online cases.} Although offline can serve as a measurement of agents' ability to some extent, it's better if we adopt online environment to allow different paths and allow some "explorations" and errors of the agent on the website.

%\subsubsection{Limitations of GPT-4V}
\label{sec:problems}
% \noindent\textbf{SR by Task Difficulty}
% We group tasks by task difficulty approximated with the number of actions for a task in offline evaluation. Based on the results in Figure~\ref{fig:sr_difficulty}, \lmmweb\textsubscript{Oracle} can achieve about 80\% % success rate on simple tasks. \lmmweb\textsubscript{Choice} also achieve about 60\% success rate on simple tasks. 


% And it's often the cases the model is quite certain that elements without bounding boxes are highlighted with bounding boxes, and there is a letter as its label. Alternatively, it is given an incorrect bounding box\boyu{Boyu: what does this sentence mean?}. Finally, the model does not understand relative positions \boyu{"well"?} and artificially \boyu{"this word seems redundant"} added labels, resulting in it often choosing the label of another nearby element as its answer. \boyu{Boyu: one senario not mentioned here is that the model link the bounding box to a non-exist or far away letter. Which is not caused by the "relative postion" stuff.}



% \begin{itemize}
%     \item \textbf{Wrong Action Generation}: \gptv\ can not generate description about the target element. The model directly failed in the first step action generation. The model's understanding ability seems suffered from the annotations in the images, compared to the results of Oracle, which revealed the potential for action generation. This is reasonable because the annotations always cover up some information of the image to a certain extent, no matter what.
%     \item \textbf{Make up annotation and image choices}: The model erroneously claims that certain elements are highlighted with bounding boxes and are labeled with uppercase letters, which actually are not. Probably because the model is overruled by LLM.
%     \item \textbf{Fail to Link Target Element to Correct Label} Although the model can recognize bounding boxes, it failed to link it to the correct labels adjacent to the bounding boxes. There are two common cases in this category. One is the model link the highlighted element to a label of its nearby element because it cannot have an accurate sense of relative positions. The other one is that the model makes up a wrong label(which is far away or non-existing) for the element, which is also probably due to LLM's overrule.
% \end{itemize}



% \subsection{The First One or the Final One}

% % \boyuan{Boyu: BTW @Boyuan, I just realized that our exp3 was inputting the (almost) whole screenshot, which suffers from the image resolution problem of WebUI. The final score of API-High should be even better.}

% emppiracally find that the first one works better for \ourmethod

% if final one,

% decent action generation

% follow the generate then discriminate approach in \ourmethod . It's working well






==> sec/5_analysis.tex <==
% \section{Analysis}

% \subsection{Improving Vision Prompting}
% \label{exp:image_prompt}

% In this section, we discuss how important the prompt is for leveraging image information.

% \begin{table}[ht]
% \centering
% \begin{tabular}{|l|ccc|}
% \hline
%  & \multicolumn{3}{c|}{Cross-Task}  \\
%  & Ele. Acc & Op. F1 & Step SR   \\
% \hline
% Baseline Prompt & 43.4 &  &  \\
% \hline
% Inductive Prompt & 53.08 & 90.69 & 50.64  \\
% \hline
% \end{tabular}
% \caption{Perfomance on GPT-4Vision with different prompts}
% \end{table}
% \label{tab:image-prompt}

% Table~\ref{tab:html_image} shows the performance difference between a model with a minimal changed prompt and a carefully designed vision prompt. According to the results, the model experienced significant performance gains with carefully designed prompts that specifically instructed the model on how to leverage image information. 

% \subsection{Image Annotation Error Analysis}
% \label{sec:hallcunication-analysis}
% \begin{figure}[t]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \includegraphics[width=1\linewidth]{figs/hallucination_analysis.pdf}
%     }
%     \caption{
%     Hallucination Error Cases Analysis
%     }
%     \label{fig:hallucination_error_analysis}
%     %\vspace{-15pt}
% \end{figure}


% \boyu{Boyu: Should consider remove hallucination. It's not only hallucination problem. wrong  generation and linking to relative label is not hallucination. Or at least the action generatoin.}

% To further explore \gptv's weakness in understanding image details and relative spatial location\boyu{Boyu:Not sure have you and where did you mention this two. And how to organize the stuff.}, we sample 100 predicted actions and perform error case analysis to investigate the reason for hallucination failures shown in the offline experiment. Our observations indicate that the model predominantly exhibits the following types of errors:

% \begin{itemize}
%     \item \textbf{Wrong Action Generation}: The model directly failed in the first step action generation. The model's understanding ability seems suffered from the annotations in the images, compared to the results of Oracle, which revealed the potential for action generation. This is reasonable because the annotations always cover up some information of the image to a certain extent, no matter what.

%     \item \textbf{Make up annotation and image choices}: The model erroneously claims that certain elements are highlighted with bounding boxes and are labeled with uppercase letters, which actually are not. Probably because the model is overruled by LLM.
    
%     % \item \textbf{Make up Image Choices} Even though the target element is not annotated, the model still claims it is highlighted with a bounding box and has an uppercase letter label.
    
%     % Model can not recognize the bounding box with the target element 
    
%     % \boyu{[Boyu: (if it has. But the model dont see the highlight so predict NA)]}or make up bounding boxes(highlights) \boyu{Boyu:(If it doesnt have. But the model say there's a bounding box with alabel)}. \boyu{[Boyu: It's maybe will be due to that the model predicted the true element, but the true element is not in the choices. Then it assume there's a bounding box of it.]}
%     \item \textbf{Fail to Link Target Element to Correct Label} Although the model can recognize bounding boxes, it failed to link it to the correct labels adjacent to the bounding boxes. There are two common cases in this category. One is the model link the highlighted element to a label of its nearby element, because it cannot have a accurate sense of relative positions. The other one is that the model makes up a wrong label(which is far-away or non-existing) for the element, which is also probably due to LLM's overrule.


    
%     % Although the model recognized the target element, it gives a wrong label as its choice. Some are caused by the model's weakness in recognizing relative positions in the image, hence it linked the element to another nearby element. While some are directly linking the element to a non-existing or far-away letter.
    
% \end{itemize}

% From our observation and counting, the errors mainly comes from the affected action genration and the hallucination when it comes to large and complex web senarios. The web elements are dense arranged, so the image annotations inevitably covers up some content of the screenshots. And it's often the cases he model is quite certain that elements without bounding boxes are highlighted with bounding boxes, and there is a letter as its label. Alternatively, it is given an incorrect bounding box. Finally, the model does not have a good understanding of relative positions and artificially added labels, resulting in it often choosing the label of another nearby element as its answer.


% % \subsection{The First One or the Final One}

% % % \boyuan{Boyu: BTW @Boyuan, I just realized that our exp3 was inputting the (almost) whole screenshot, which suffers from the image resolution problem of WebUI. The final score of API-High should be even better.}

% % emppiracally find that the first one works better for \ourmethod

% % if final one,

% % decent action generation

% % follow the generate then discriminate approach in \ourmethod . It's working well

\section{Qualitative Study}
\label{sec:qualitative_study}

% \boyu{Boyu is working on this part. The language is not refined. Still is adding content.}

\subsection{GPT-4V is a Powerful Web Action Planner}
\label{4visgoodplanner}
Instead of textual similarity matching, cases in our experiment show that \gptv\ is indeed doing webpage examining, understanding, reasoning, and decent planning.

In \ourmethod , we explicitly instruct the model analyze the webpage and previous history to make it understand the environment and history. Fig. \boyu{[Boyu: Ref the Truck case]} shows its impressive ability in doing this. This query is challenging because two crucial information had not been recorded in the history, namely the filled "Drop-off Date" and the clicked "No" button. However, \gptv\ found this two evidences from its close examination, and hence made the right decision.

\boyu{"Still lack some cases to show the reasoning"}


During action generation, \gptv could not only determine the correct current step, but also the subsequent actions. Fig. \boyu{[Boyu: Find a case GPT4V directly chose several element and give corresponding actions. There are a lot]} shows that \gptv\ directly gives a serious actions in the webpage, even we had emphasize it only should generate only the next action. And what's even surprising is that it could even foresee the approximate next steps in later webpages. In the case of Fig. \boyu{[The bestbuy spearker case]}, it suggested not only the current step in the homepage, but also the later steps in later sections. And it generated the whole plan to satisfy every aspect of the task, even if it is only a start stage.

(also mention this in the knowledge)



\subsection{Awareness of Error Correction}

\boyu{Boyu: Maybe we can merge this into 5.1}

Fig. \boyu{ref the mobile phone number case} is a "wrong" answer in offline, but it reflects that the model has an awareness of correcting the errors caused by previous steps.

It's more often in online, and is more crucial in online. 

A key difference between offline and online is that, the previous actions are not golden annotated actions. Here it does not only mean simple cases that involves interchangeable steps, but also mean the previous actions may have caused fatal errors or even totally wrong, which lead to a webpage that is far away from the goal.

Hence online testing really requires the model to have an awareness of correcting its errors and move it to the correct direction.


\subsection{Knowledge Requirement}

\boyu{GPT4V is a knowlegeable model, which is a huge advantage compared to MindAct}

\gptv\ is undoubtedly a knowledgeable model. That's partly it has superior planning ability showed in \ref{4visgoodplanner}. On the other hand, some tasks indeed require specific knowledge, which is hard for MindAct-like models.

\boyuan{
1.Smaller models inherently possess less knowledge; \\2. the fine-tuning process further cause catastrafic forgetting; \\3.The model also are not able to generate intermediate thoughts
}
The fine-tuned model tends to serve as a specifialist model to convert low-level tasks into executable actions (sort like semantic parsing)

\subsection{Challenges of Textual Referring}
\boyu{Boyu: this is a minor point, consider removing this. and directly refer these images when talking about the limitation of SeeAct\_{Text\_Choice}}

identical element, impossible to clarify. Empirically find that it tends to choose the first one. 

misleading by the textual content of options , need clarify these.

the image annotation potentially can cease this problem, but not doing well though due to the complexity of the web env and hallucination issue.

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/case_study/test_template.pdf}
%     \caption{The predicted element is located at a neighboring element of the target element.}
%     \label{fig:neighbor-element}
% \end{figure*}
% \newpage


\subsection{Unlearned Human Habits}
\boyu{boyu: Merge this into section 4 the weakness of GPT-4V}
\boyu{Boyu: Still need to consider more weakness points of GPT-4V}
dont click suggested items in drop down

forget to confirm.

Have awareness. But if think from scratch again. It fails

% \subsection{Insufficient Information of High-Level Tasks}

% \boyu{Boyu: this is a minor point, consider removing this}

% sometimes the task is too high-level, which demand the models consider how to handle ambiguous steps. It's often the case the website require an option or a input area that is not specified in the task intent.


\subsection{Action Series Variation}

To complete a task, the actions always can be varied. A basic while fatal issue of offline evaluation is that it suffers a lot from interchangeable steps. For example, for the filling process of every form can be various. \boyu{ref the AA form}. Additionally, some webpages have several link leading to the same next page, which should be all considered as correct element.  \boyu{ref the drug.com case}

A more common case in online testing is that, the action series can be totally various in a webpage-level aspect, not only the actions within a single webpage. For example, the agent may forget or fail to execute an action, but it may fix it in later steps. To conclude, the action can be far deviate from the annotated action paths. \boyu{ref the previous Fig.6 or other online cases.}

Although offline can serve as a measurement of agents' ability to some extent, it's better if we adopt online environment to allow different paths and allow some "explorations" and errors of the agent on the website.


% And this is even the case when it comes to realistic websites, where the order between webpages can also various.  



\boyu{basic: interchangeable action order

Higher: Totally different path, and allow exploration.}












% \boyu{[Boyu's adding:\textbf{Inventing Textual or visual description} Sometimes invent textual content or visual content description, which are crucial for automatic locating, especially the textual content. Notice this case happens not only in image annotation style]}

% \boyuan{Classify errors base on the yann posted paper and add a bar chart for error analysis}



% \subsection{One Turn or Multiple Turn}

% When humans are tasked with drafting documents, especially first drafts, and are simultaneously required to adhere to stringent grammatical and logical structures, the flow of creativity can be hindered. Contrastingly, if the initial focus is on freely expressing thoughts and ideas without concern for grammatical precision, a wealth of innovative concepts tends to emerge. These raw, unfiltered thoughts can later be refined and structured into coherent content. With this in mind, we consider two experimental settings:
% \begin{itemize}
%     \item \textbf{Single-Turn} In this setting, the model is tasked with generating both the preliminary ideas and the polished, final response in one inference turn.
%     \item \textbf{Two-Turn} This setting split the formatting step into a seperate second turn, whcih allows the model to general richer intermediate thoughts with constraints.
% \end{itemize}

% In Table~\ref{tab:one_multiple_turn}, model performance varies significantly between single-turn and two-turn setting. This variance leads us to hypothesis multi-turn method may be more conducive to generating richers intermediate thoughts by preventing the model from being hindered by formatting constraints.

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|ccc|}
% \hline
%  & \multicolumn{3}{c|}{Cross-Task}  \\
%  & Ele. Acc & Op. F1 & Step SR   \\
% \hline
% Single-Turn & 33.92 &  &   \\
% \hline
% Two-Turn & 53.08 & 90.69 & 50.64  \\
% \hline
% \end{tabular}
% \caption{Performance difference with one or two turns}
% \end{table}
% \label{tab:one_multiple_turn}



% \subsection{GPT-4V Error Case Study}
% In this section, we will analyze the error cases in the action generation step, which can indicate the ability limit of GPT-4V.

% \boyu{[Boyu: One interesting error is that the gpt4v is lacking some knowedge, for example some geography knowledge. Some tasks, as only given the highlevel intent, requires profound knowledge to understand how to accomplish. So I do believe we should subdive the high-level intent into  low-level and detailed actions for speciallized model. ]}

% \boyu{[Boyu's Comment: two common cases: 1. forget to confirm after typing into search box. 2. Tend to directly put all the things into search box and search]}



% \paragraph{Preference for Search Box}

% \paragraph{No Enter after typing}




% \subsection{Hybrid Referring}
% Considering advantages and limitations of each referring method, we propose to ensemble different methods to achieve a better performance. Although directly letting models refer to webpage elements through labels around the bounding box does not lead to a decent performance, referring with image annotation still has potential to help resolve ambiguous choices in the Textual Choices setting when webpages are not too complex.

% So we conduct experiments, introducing image annotation into the final round of Textual Choices setting, where the agent only need to pick a final answer from few likely elements predicted by the previous inference batches. 

% As for the final round inference, the model will be given only two or three elements. Hence we merely add two or three labels and bounding boxes as image choices. We compare results from the following three settings regarding whether we provide text choices and whether we add bounding boxes and labels to the input screenshot for visual identification. 
% \begin{itemize}
%     \item \textbf{Only Text Choices:} the original setting.
%     \item \textbf{Only Image Choices:} change to the Image Annotation setting.
%     \item \textbf{Both Text and Image Choices:} take annotated screenshots as input, while still provide text choices.
% \end{itemize}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|ccc|}
% \hline
%  & \multicolumn{3}{c|}{Cross-Task}  \\
%  Choice Style& Ele. Acc & Op. F1 & Step SR  \\
% \hline
% Text & 50.61 & 85.37 & 46.67  \\
% \hline
% Image & 48.14 & 89.75 & 45.45  \\
% \hline
% Text+Image & 54.32 & 88.64 & 51.31  \\
% \hline
% \end{tabular}
% \caption{Perfomance on GPT-4V with different prompts in the final round. \boyuan{Change chart}}
% \end{table}
% \label{tab:final_round}



% \subsection{Image Annotation Type Impact}
% The image annotation type in Section~\ref{referring:exp2} is not limited to our implementation of bounding boxes and alphabetical labels. There exist multiple ways to apply image annotation. 

% \begin{itemize}
%     \item \textbf{Bounding Box} Adding bounding boxes around candidate elements listed in options can specifically locate elements on the webpage instead of relying on GPT-4V's capability of finding the text-image alignment.
%     \item \textbf{Masking} Masking can make the element more visible than solely bounding box
%     \item \textbf{Labels} Labels can specifically highlight 1-to-1 alignment between webpage elements and text choices.
% \end{itemize}

% \subsection{GPT-4V Failure Case Analysis}
% Although GPT-4V shows great ability in recognizing objects or texts on web pages well, it may still make mistakes that can't see elements very obvious to the human eye, as shown in Figure~\ref{fig:error-correction-case}. In this figure, the target element is "Air Quality", which is very obvious to humans. However, GPT-4V's generation shows there is no visualizable element with a function to check air quality on the screen.


==> sec/bck_1_intro.tex <==
\section{Introduction}
\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics[width=1\linewidth]{figs/vlm_teaser.pdf}
    }
    \caption{
    Comparison of web navigation task strategies: GPT-4V uses webpage screenshots, while traditional models rely on HTML text. A segment of a webpage screenshot corresponds to a significant amount of tokens for its HTML text counterpart, even when CSS is excluded.\hs{some thoughts on the figure: the upper part and the bottom part might be more separated; the openAI logo might be removed.}
    }
    \label{fig:teaser}
    %\vspace{-15pt}
\end{figure}
Recent advancements in Vision Language Models (VLMs) have marked a significant leap forward in multimodal scenarios~\cite{Li2023MultimodalFM, yang2023dawn}. Emerging research is increasingly leveraging image representations to empower web navigation tasks~\cite{Li2022SpotlightMU, Shaw2023FromPT, Furuta2023MultimodalWN}. 
Unlike text-only models that can only ground on HTML text within limited token length, VLMs leverage condensed, visual-rich image representations, preserving crucial visual cues and facilitating more nuanced web agent interactions. For instance, a small segment of a webpage image can encapsulate what thousands of HTML tokens attempt to convey. As illustrated in Figure~\ref{fig:teaser}, a screenshot segment worthing merely \num{595}~\footnote{Calculated with OpenAI Vision pricing calculator: \url{https://openai.com/pricing}} text tokens needs \num{43215} HTML tokens to convey its meaning. 




% Webpage image shows several advantages as the representation to ground web agent comparing with HTML text: (1) Efficient Representation: Images provide a condensed, information-rich format that circumvents the verbosity and context limitations inherent in extensive HTML texts. (2) Preservation of Visual Information: Crucial visual information is retained, enhancing comprehension and interpretation. (3) Enhanced Webpage Interaction: Designed for human engagement, webpage environments convey a wealth of actionable data, beneficial for web agents in decision-making processes. As shown in Figure~\ref{fig:teaser}, even a small chunk in the webpage screenshot image corresponds to a lengthy HTML text with 43,215 tokens even after removing all CSS codes for visual features. However, the corresponding image screenshot only need 595~\footnote{Approximation via OpenAI \href{https://openai.com/pricing}{Vision pricing calculator}} text token after projecting the corresponding image. 

Fine-tuning VLMs on annotated datasets has shown promise for web navigation and mobile UI comprehension, as demonstrated by WebAgent~\cite{Gur2023ARW}, WebGUM~\cite{Furuta2023MultimodalWN}, and Pixel2UI~\cite{Shaw2023FromPT}. Despite their potential, these models often struggle with generalizing to new, unseen distributions. In contrast, foundation models such as LLaVa~\cite{Liu2023VisualIT} and MiniGPT4~\cite{Zhu2023MiniGPT4EV}, Bard-Vision offer better generalization but fall short in complex web navigation tasks.
% Significant advantages of grouding agents on webpage images have been intensively demonstrated by previous works on both web navigation~\cite{Shaw2023FromPT} and mobile UI understanding~\cite{Li2022SpotlightMU, Furuta2023MultimodalWN} by fine-tuning vision-language models in annotated training data. Fine-tuning models, such as WebAgent~\cite{Gur2023ARW}, WebGUM~\cite{Furuta2023MultimodalWN}, and Pixel2UI~\cite{Shaw2023FromPT}, shows signiciant potential as web agents taking advantage of the digital nature of website environments, which provide large amount of data and live feedbacks. However, they still suffer from bad out-of-distribution generalization. 

% Although generalist models, like LLaVa~\cite{Liu2023VisualIT}, MiniGPT4~\cite{Zhu2023MiniGPT4EV} have the advantages of good generalization ability, their potential in this sphere remains underexplored, due to the inadequacy of model performance when dealing with tasks with complexity of web navigation. 

The advent of the GPT-4V model brings new capabilities to the field. While many works have already shown its strong ability among a wide range of tasks and scenarios, a detailed quantitative analysis of its application to web navigation is pending. This paper investigates GPT-4V's proficiency in web navigation, providing empirical benchmarks against current solutions. We explore the challenges in referencing specific webpage elements, which is the key to deploying practical web agents—and propose innovative solutions. Our experiments reveal that with optimized referencing techniques, GPT-4V based agents achieve superior performance on the Mind2Web benchmark.

% However, the advent of GPT4-Vision model demonstrates remarkable performance across multiple tasks. While GPT4-Vision has showcased its versatility in varied contexts~\cite{yang2023dawn}, a comprehensive, quantitative analysis of its efficacy in web navigation tasks is still pending. 
% In this work, we want to explore GPT4V's ability in web navigation task and provide quantative results to benchmark its performance by cpmparing with other exsiting solutions. In our experiments, we find GPT4V are powerful at web navigation tasks by generating textual description about next step action. However, it's still challenging to models to refer to specific webpage elements, which is the essential steps towards applying GPT4V for practical web agent. The referring process requires a handle to bridge text and image. One potential solution is provding textual description of webpage elements and let GPT4 to directly refer to them by selecting textual choice, which leads to our solution in Section~\ref{referring:exp3} and Section~\ref{referring:exp4}. Another direction is adding annotation, like labels for elements, to image so that GPT4V can refer by generating the corresponding label of webpage elements, which leads to our solution in Section~\ref{referring:exp2}. To measure GPT4's performance limits if we can provide a perfect referring method, we conduct two-way annotation and find the large margin between existing referring methods and a prefect referring method. 

% We further discover the limitations in evaluating model's success rate at completing a whole task using offline dataset. To solve these limitation, we propose live evaluation on real websites and develop tools to enable that. 

Additionally, we explore the limitations of using offline datasets for evaluating task completion and propose a novel, live evaluation framework on actual websites. This allows for real-time assessment and addresses the shortcomings of static simulated environments in Mind2Web. \boyuan{[add some conclusion]}

To summarize, our contributions are threefold:
\begin{itemize}
    \item We present the first quantitative analysis of GPT-4V in web navigation, establishing a performance benchmark via human evaluations.
    \item We pinpoint the challenges associated with webpage element referencing and propose three solutions underpinned by experimental findings and a comprehensive analysis of their strengths and limitations. With proper referring, our web agent based on GPT-4V achieves the best performance on Mind2Web.
    \item We introduce a novel online evaluation framework for web agents, enabling real-time performance assessments on live websites, thus overcoming the constraints of traditional simulated evaluations.
\end{itemize}

==> sec/bck_2_formulation.tex <==
% \section{Web Navigation Task Formulation}
% \section{\hs{Preliminaries}}
% \section{Background}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/vlm_web_figure2_v2.pdf}
%     \caption{An example for element referring with three different methods.\hs{I feel this figure is very confusing..I am expecting to see `three methods' with index for each. Also, do you mean doing an ensemble at the bottom left part? B/C/D/E are already filled in previous steps, right? or they are candidates for this step?}}
% \end{figure*}
% \label{fig:main-figure}
% \noindent \textbf{Task Formulation.} Web navigation \cite{deng2023mind2web, Yao2022WebShopTS, Zhou2023WebArenaAR, liu2018reinforcement} is defined as a sequential decision-making problem where agents interact with a web-based environment to accomplish tasks described in natural language. Specifically, given a high-level task described in natural language, the agent's objective is to accomplish this task by generating a sequence of web navigation actions, each comprising an element of a webpage for interaction and the requisite operation to be executed on the target element. To complete the given task, the agent needs to be grounded in a web environment. The observation from the web environment is HTML text for text-only language models and webpage screenshots for vision-language models.

% At each step of decision-making, the agent is tasked with generating an action that can be converted into a browser event. The action generation is conditioned on the task description, the history of actions that have been taken, and the observation from the environment. Each web navigation action encompasses: (1) \textbf{Webpage Element}, which must be as precise as a specific node ID on the webpage to ensure accurate element localization. (2) \textbf{Operation Type}, the kind of action operation in predefined action space, like "CLICK". (3) \textbf{Operation Value}, indicating the necessary input for the web navigation action. 

% For example, in Figure~\ref{fig:teaser}, the agent's task is "Rent a Truck" within the web environment of Truck Rental website. In vision-language models, such as GPT-4V, the observation comprises a screenshot from the truck rental website's homepage. For text-only models like GPT-4V, the observation is limited to the HTML text used to rendering the screenshot. As illustrated in Figure~\ref{fig:teaser}, a relatively small portion of the webpage screenshot necessitates a substantial volume of HTML text for its generation.

% %~\\
% \noindent \textbf{Challenges.} 
% Webpage environment usually contains thousands of elements, leading to an action space with high complexity and a context exceeding the max token length of language model. Two-stage strategy is taken to deal with this challenge by firstly selecting candidate elements and action prediction based on the selected context. \citet{deng2023mind2web} utilize a cross-encoder for element ranking and \cite{Zhou2023WebArenaAR} 

% Evaluation is also a major challenge here. An ideal benchmark should be both diverse enough with numerous websites, tasks across numerous domains and can provide dynamic interaction with the web agent. Although signiciant efforts has been invested in building benchmarks, they are far from a ideal benchmark. Dynamic benchmarks, like WebArena, can support interaction with web agent, but fall short in environment diversity and resemblence to real websites. In contrast, static benchmarks, like Mind2Web, has the advantage of diversity, but can not support interaction with agents.

% \hs{also consider describing the evaluation challenge with limitations of existing datasets, which will lay the groundwork for introducing your live evaluation framework?}

% \subsection{Challenges}

% There are two kinds of capabilities and challenges of GPT-4Vision that's vital for leveraging GPT-4Vision in web navigation tasks: \textbf{Action Generation} and \textbf{Element Referring}. 
% \paragraph{Action Generation}
% During each step of action generation, GPT-4Vision initially produces a description for the subsequent action. This description encompasses both a high-level strategy and detailed, low-level steps. Mostly, these steps will be preceded by intermediate thoughts. The quality of generation at this stage represents the upper limit of the model's capability in web navigation tasks. In Section~\ref{sec:upper_bound}, we implement human annotation to manually determine whether the generated intermediate thoughts and action descriptions adequately capture the essence of the intended target element and action.

% \paragraph{Element Referring}
% Creating an accurate action description, which encompasses the details of the targeted action, doesn't necessarily equate to a correct web browser event. Web navigation tasks demand precise references to webpage elements, enabling the model to execute specific actions within the browser. Following the action generation, there is an additional step of element referencing where the model must accurately identify a specific element on the webpage. We will explore various potential approaches to this element referencing in detail in Section~\ref{sec:referring}.



==> sec/bck_3_experiments.tex <==
\section{Experiments}


\subsection{Dataset}
\label{sec:dataset}

Mind2Web~\cite{deng2023mind2web} is a recent comprehensive dataset encompassing over \num{2000} web navigation tasks with annotated actions across \num{137} varied websites spanning \num{31} distinct domains. This dataset is designed to evaluate the generaliz abilities of web agents across different tasks, websites, and domains. 

% In Mind2Web, the operation space is defined by three actions: "CLICK", "SELECT", and "TYPE". Operations like "Hover" and "Enter" are not explicitly listed, as they can be achieved using the three primary operations. The operation value is contingent on the type of operation. For a "CLICK" operation, the default value is "None". In contrast, for "TYPE" and "SELECT" operations, the value corresponds to the input for the respective element.

To provide webpage screenshots for each action, we align the screenshot metadata from the Mind2Web raw dump with each corresponding action. However, due to errors in capturing during dataset construction, not all screenshots are usable. We conduct a manual selection to ensure that (1) the screenshot is correctly rendered and (2) the target element is visible in the image. Given the limited quota of GPT-4V inferences\footnote{There is rate limits for both OpenAI GPT-4V API and ChatGPT WebUI}, for each split (cross-task, cross-website, cross-domain), we randomly select 30 tasks for experiments.

%our experiments are conducted on a randomly selected subset of 30 tasks from each split.


\subsection{Baselines}
We access GPT-4V via the ChatGPT Web UI and compare the model with the following baselines:
% \hs{Our focus is GPT-4V, right? the following methods are just `Baselines', right? if so, we could change the title to `Baselines'.} 
% \hs{We access GPT-4V via the ChatGPT Web UI and compare the model with the following baselines:}

\noindent \textbf{MindAct.}
\citet{deng2023mind2web} propose a two-stage framework to deal with the complexity of the web environment by firstly ranking top-k elements with a trained cross-encoder and then performing action generation with different language models. The cross-encoder is based on DeBERTa (base) with 86M parameters trained on the training set of Mind2Web. It achieves 88.9\% / 85.3\% / 85.7\%  Recall@50 under the cross-task, cross-website,
and cross-domain setting, respectively. In our baseline experiments\hs{what do you mean by `baseline experiments?' only this setup for baselines?}, we leverage this cross-encoder and pick top-40 ranked elements as the candidate pool for action generation.

% involving environment summarization and action generation. The first stage is \textbf{environment summarization}, where the model needs to distill raw HTML documents into task-relevant snippets. \citeauthor{deng2023mind2web} trained a cross-encoder based on DeBERTa~\cite{He2020DeBERTaDB} to rank top \num{50} elements. ~\citeauthor{Gur2023ARW} pretrained FLAN-T5 models on HTML data and performed instruction tuning for HTML summarization for this purpose. We make use of the trained cross-encoder ranker for our experiments.

% The second stage is \textbf{action generation}, where the model needs to predict actions grounded on the web environment snippet from the first stage. \citeauthor{deng2023mind2web} fine-tuned FLAN-T5~\cite{Chung2022ScalingIL} with annotated action trace in Mind2Web for action generation by selecting from the candidate elements from the first stage.
\noindent \textbf{FLAN-T5.} 
We train FLAN-T5~\cite{Chung2022ScalingIL} of three different sizes on the training data of Mind2Web to enable it to generate target actions in our defined format.

\noindent \textbf{BLIP2.} 
BLIP2~\cite{Li2023BLIP2BL} 
% \jh{Seems like the citation is not correct. This is BLIP, not BLIP-2.}
combines a FLAN-T5 language model with a CLIP~\cite{Radford2021LearningTV} image encoder, bridged by a projection layer. This model can integrate the same FLAN-T5 language model as the text-only model, ensuring consistent comparison and analysis. We freeze the image encoder for training and fine-tune the projection layer and language model. We set the resolution to image encoder resolution to 2048.

\noindent \textbf{GPT4 \& GPT3.5.} 
We also evaluate GPT3.5-turbo-0613 and GPT4-turbo-1106-preview, via access through OpenAI API. 


% For the supervised vision-language model\hs{should we also give a name to this approach? currently it looks like part of MindAct?}, we select 
% BLIP2~\cite{Li2022BLIPBL}, which integrates the same FLAN-T5 language model as the text-only model, ensuring consistent comparison and analysis. This model combines a FLAN-T5 language model with a CLIP~\cite{Radford2021LearningTV} image encoder, bridged by a projection layer. We freeze the image encoder for training and fine-tune the projection layer and language model.

% \paragraph{API-based Methods?} For off-the-shelf models, we leverage GPT3.5-turbo-0613, GPT4-turbo-1106-preview, and GPT-4V accessed via the ChatGPT Web UI.


% \subsection{Human Evaluation}
% \label{exp:human_eval}

% \hs{should we move this to `Main Results' and put it the first two paragraphs there?}

% To evaluate GPT-4V's performance cap, we first prompt the model to directly generate descriptions about the next step action without constraints of the output format\hs{what are `the constraints of the output format'? without applying our methods for element referring?}, as described in Section~\ref{sec:action-generation}. %which allows humans to extract information about the target element, the operation, and any operational values associated with it. 

% Human annotators are asked to determine whether the generated action descriptions contain adequate and valid information to derive the target webpage element, operation, and operational values. This evaluation serves as a metric for the model’s potential in web-based tasks. We ask two annotators to score each example and use the average score as the final result. We further calculate inter-annotator agreement with Cohen's Kappa Coefficient~\cite{McHugh2012InterraterRT}.
% % We perform two-way annotation \hs{what does this mean?} to label scores for each action, resulting in a Cohen's Kappa Coefficient~\cite{McHugh2012InterraterRT} of @placeholder\hs{what does this mean?}, denoting a high/medium/low agreement level among annotators. 
% Our results, as illustrated in Table~\ref{tab:main}, 
% % \hs{wrong index}
% reveal an element accuracy rate of \num{84.9}\%, significantly surpassing existing methods across all evaluated categories.


\subsection{Static Evaluation}
\label{sec:offline-eval}
We adopt the evaluation metrics utilized in Mind2Web ~\cite{deng2023mind2web}. We assess \textbf{Element Accuracy} by comparing the predicted element with the target element.
%against all target elements.
Then, we assess \textbf{Operation F1}, which is the token-level F1 score for the predicted operation comprised of action and input value. Each step of the task is independently evaluated against the provided ground truth action. %history.

Further, we also use 
% introduce two key metrics\hs{these two metrics were already used in Mind2Web, right? why ``we introduce'' here?}: 
\textbf{Step Success Rate} and \textbf{Whole Task Success Rate}. A step is considered successful if the element and the operation prediction are correct. Similarly, a task is deemed successful only if all of its steps are completed successfully. \hs{do you have whole task success rate in Table 1?} For the step-wise evaluation, we calculate the macro-average across various tasks.




\subsection{Results}

\paragraph{Human Referring Evaluation}
% We calculate inter-annotator agreement with Cohen's Kappa Coefficient~\cite{McHugh2012InterraterRT}.
% We perform two-way annotation \hs{what does this mean?} to label scores for each action, resulting in a Cohen's Kappa Coefficient~\cite{McHugh2012InterraterRT} of @placeholder\hs{what does this mean?}, denoting a high/medium/low agreement level among annotators. 

As illustrated in Table~\ref{tab:main}, LMM2Web achieves 76.4\% / 79.1\% / 84.9\%  Element Accuracy on Test\textsubscript{Cross-Task}, Test\textsubscript{Cross-Website}
and Test\textsubscript{Cross-Domain}. Human referring also achieves the best performance on Operation F1 and Step Success Rate. These performance claims GPT-4V's strong capability as a generalist web agent with a good referring method. 

\paragraph{Referring Methods Comparison}
Our experiment results, as depicted in Table~\ref{tab:main}, reveal that referring with textual choice exhibits the best performance among the three evaluated referring methods. However, it significantly trails behind the performance of human referring, indicating substantial space for improvement. Notably, referring through image annotation, while intuitively appealing, suffers from poor performance. This is primarily attributed to the limitations of GPT-4V in processing detailed image information, which will be discussed in detail in Section~\ref{sec:hallcunication-analysis}. 
% GPT-4V is capable of recognizing bounding boxes and their contents, as well as labels within images. However, it struggles with color recognition in complex webpage settings and binding labels to bounding boxes. 
Referring to attributes lies between the other two methods. The performance of this model is predominantly limited by the heuristic-based approach employed for element localization, which relies on text and type.

Despite these methods showing promise, human referring scores reveal a significant performance gap, approximately \num{30} to \num{40} points, between the existing methods and the optimal performance potential of GPT-4V. This underscores the urgency of refining the referring methods for effective web navigation using GPT-4V.



\paragraph{LMM, VLM, LLM Comparison}
In our supervised learning experiments, we employed FLAN-T5 as the text-only language model and BLIP2 as the Vision-Language Model (VLM). BLIP2 integrates the FLAN-T5 language model with a CLIP encoder and a projection layer, facilitating the conversion of image representations into text tokens. The selection of these models was aimed at providing a fair comparison to demonstrate the impact of the vision module in the VLM. 
According to the results presented in Table~\ref{tab:main}, the base size models show that BLIP2 surpasses T5 in cross-task and cross-website performance but lags behind in the cross-domain split. For the large and XL models, T5 consistently outperforms BLIP2. However, these findings alone are insufficient to 
% \hs{this message seems like a negative msg, and needs to be rephrased. what do you think the problems are and what potential solutions could be?}\boyuan{[BYZ:Have added one paragraph to explain reasons]} 
conclusively determine whether Vision-Language Models (VLMs) or text-only Language Models (LLMs) are more suitable for fine-tuning web navigation tasks. 

There are several potential reasons behind the our BLIP2 bsaed model. Firstly, although we ensure the screenshot in the three test splits are flawless, the ones in the training set may still have errors, like rendering failures and the annotators may take the screenshott at a wrong time. Secondly, the CLIP model as image encoder is not good enough for attending to image details as studied in ~\citet{shen2021much}. Our web navigation task is demanding on image detail understanding. \boyuan{BOYUAN: I am Training new batch of BLIP2 with 2048 resolution (640 previously) seems to shows the advantage of BLIP2 compared with FLAN-T5}


GPT-4V shows significant advantage over its corresponding LMM (GPT4 and GPT3.5) using the proper referring method of textual choices. The advantage can be more obvious when comparing LLMs' performance with LMM with human referring.


\paragraph{SOTA model discussion}
The performance achieved by GPT-4V with human referring set a high benchmark, showcasing the best performance that GPT-4V can potentially reach. This includes approximately 80\% element accuracy and an 80\% success rate for single actions. Such performance significantly surpasses all existing solutions, particularly regarding generalization to new websites and domains. From this, it's evident that GPT-4V is a strong model for web navigation tasks.

Moreover, the most effective referring method we investigated also yields the best results in cross-website and cross-domain splits. In the cross-task split, our method falls short of fine-tuned models at large and XL sizes but surpasses all other methods. However, even this performance still significantly trails behind that of the human referring method. With further improvement in referring methods, GPT-4V has the potential to demonstrate even more impressive performance, possibly outperforming fine-tuned models in in-domain data. Nonetheless, the potential of fine-tuning models for in-domain scenarios is substantial, especially considering the vast amount of data available from millions of websites.

\section{Online Evaluation on Live Websites}
\label{sec:online_eval}


\boyuan{[Consider removing this to introduction and online evaluation experiments into the experiment section]}
Step-wise performance provides a good evaluation of the models' ability to ground to web environments and generate a single action. However, these evaluation is not enough to assess agents' ability to complete whole tasks on websites. An ideal benchmark should possess the following properties: (1) Broad coverage of diverse website environments across various domains; (2) Diverse tasks that can challenge multiple aspects of the model's capability; (3) Dynamic environment to handle action sequence variability and provide interactions and feedbacks to agents.

\subsection{Challenges}
Despite substantial efforts to develop such an ideal benchmark, current benchmarks still fall short. Webshop~\cite{Yao2022WebShopTS}, miniWoB++\cite{liu2018reinforcement}, and WebArena\cite{Zhou2023WebArenaAR} create local website environments to facilitate dynamic interactions. However, the engineering work required to build these web environments is extensive, leading to a limited number of websites and insufficient task diversity. The simulated environments are also not close enough to real websites. 

Mind2Web~\cite{deng2023mind2web} fulfills the first two criteria by dumping webpages from numerous websites across a wide range of domains and annotating a large set of diverse tasks with annotated traces. However, Mind2Web only offers a static environment through webpage dumps. This static approach has two primary limitations:
\begin{itemize}
\item \textbf{Action Sequence Variability} A single task can be completed through multiple potential action sequences, such as altering the order of actions, as depicted in Figure~\ref{fig:online-eval}. In a static environment, evaluations can only compare the generated action sequence with a single predefined target sequence.
\item \textbf{Lack of Environment Interaction} Interactions with the environment are critical for web agents to correct errors and explore options to find the optimal solution, as illustrated in Figure~\ref{fig:online-eval}. Static environments lack this interactive component.
\end{itemize}


\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics[width=1\linewidth]{figs/online_eval_figure.pdf}
    }
    \caption{
    Example to show the difference between static environment and an online evaluation 
    }
    \label{fig:online-eval}
    %\vspace{-15pt}
\end{figure}

\subsection{Online Evaluation}
To provide an ideal benchmark, we propose online evaluation on live websites using an automatic testing tool~\footnote{We will release the source code of this tool}. This tool can convert predicted elements, actions, and values into corresponding executable browser events on live websites using Playwright~\footnote{\url{https://playwright.dev/python/docs/api/class-playwright}}.

We conduct online evaluation on the same tasks subset sampled in Section~\ref{sec:dataset}. To ensure the ethics of experiments, we only conduct online evaluation experiments on licensed websites in three test data splits, allowing small-scale automatic testing. We record web agents' traces during evaluations, which will be released to encourage further research. We closely monitor agent behaviors to prevent any potentially harmful behavior, such as state-changing actions. Notably, no harmful behavior was triggered throughout our online experiments.

We make the following effort to ensure the comparison between online evaluation and static evaluation is fair. Firstly, we provide the same URL link to the website where the static webpage dumps were generated in Mind2Web. Also, some tasks are time-sensitive, we rewrite these tasks to ensure they have the same difficulty and are still valid when we conduct online evaluations.

\subsection{Evaluation Result}

We run online evaluation on in total 50 tasks randomly sampled from the whole test set since we are not able to run on some websites limited by usage license. We aggregate performance on these 50 tasks to alleviate the randomness in small-scale experiments. 

Table~\ref{tab:online_evaluation} shows the performance difference among the whole task success rate in a static environment and real-time live websites capable of providing feedback from the environment.

\subsection{Case Study}

GPt-4V based web agent shows some interesting ability during online evaluation.
Web agents demonstrates promising abilities that can not be obeserved on static environemnt during online evaluation. 

\paragraph{Error Correction}

As shown in the left half of Figure~\ref{fig:error-correction-case}, model forget to fill all required input fields
The model based on GPT-4V can correct errors in previous actions and trace back to the previous webpage to complete tasks, as shown in Figrue~\ref{fig:error-correction-case}.
\begin{figure*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics[width=1\linewidth]{figs/online_cases.png}
    }
    \caption{
    This example shows the model's capability for error correction
    \boyu{[A draft, still need consideration and revisement]}\boyu{[The screenshot of 4 and 5 is incorrect, forget to set 50, remember to re-capureture]. 
    BTW, remember there is a wrong arrow from "6"}
    }
    \label{fig:error-correction-case}
    %\vspace{-15pt}
\end{figure*}


\paragraph{Exploration to find optimal path}
A dynamic environment allows the model to explore and experiment freely within the webpage, thereby discovering the right path, as shown in the lower part of Figure~\ref{fig:error-correction-case}.

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{|l|lll|lll|lll|}
%     \hline
%          &\multicolumn{3}{c|}{Cross-Task}  &\multicolumn{3}{c|}{Cross-Website}  &\multicolumn{3}{c|}{Cross-Domain} \\
%          & Off-0& Off-1 & On & Off-0& Off-1 & On & Off-0& Off-1 & On  \\
%          \hline
%          MindAct&&&  &&&  &&& \\
%          \hspace{1em}-T5-XL&\num{3.33}&\num{26.7}&  &\num{3.33}&\num{20.0}&  &\num{3.33}&\num{13.3}& \\
%          \hspace{1em}-GPT-4&\num{3.33}&\num{13.3}&\num{11.8}  &\num{0.0}&\num{10.0}& \num{21.4} &\num{0.0}&\num{13.3}&\num{36.4} \\
%          \hline
%          % GPT-3.5&0.0&6.7&  &0.0&6.7&  &0.0&6.7& \\
%          % \hline
%          LMM2Web&&&  &&&  &&& \\
%         \hspace{1em}-TC &&& &&& &&&\\
%         \hspace{1em}-Human &&& &&& &&&\num{34.5}\\
%          % \hline
%          % FLAN-T5-XL&&  &&  && \\
%          % \hline
%          % EXP3&&  &&  && \\
%          \hline
%     \end{tabular}
%     \caption{Whole task success rate tested in both static environment (off) and online environment (on). Off-0 and Off-1 refers to tolerance for error by zero or one action step.}
%     \label{tab:online_evaluation}
% \end{table*}

% \begin{table*}[t]
% \centering
% \small
% \tabcolsep 3.5pt
% \renewcommand\arraystretch{1.0}
% \begin{tabular}{lccccccccc}
% \toprule
% \multirow{2}{*}{} &
% \multicolumn{3}{c}{Cross-Task} &
% \multicolumn{3}{c}{Cross-Website} &
% \multicolumn{3}{c}{Cross-Domain} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
%   & Off-0& Off-1 & On & Off-0& Off-1 & On & Off-0& Off-1 & On \\
% \midrule
%  FLAN-T5-XL&\num{3.33}&\num{26.7}&  &\num{3.33}&\num{20.0}&  &\num{3.33}&\num{13.3}& \\
% GPT4 &\num{3.33}&\num{13.3}&\num{11.8}  &\num{0.0}&\num{10.0}& \num{21.4} &\num{0.0}&\num{13.3}&\num{32.1} \\
% LMM2Web\textsubscript{Human} &&&&&&&&&\num{54.5}\\
% \bottomrule
% \end{tabular}
% \vspace{-5pt}
% %\captionsetup{width=0.95\textwidth} 
% \caption{Whole task success rate tested in both static environment (off) and online environment (on). Off-0 and Off-1 refers to tolerance for error by zero or one action step.}
% \label{tab:online_evaluation}
% \end{table*}

\begin{table}[t]
\centering
\small
\tabcolsep 3.5pt
\renewcommand\arraystretch{1.0}
\begin{tabular}{lccc}
\toprule
% \multirow{2}{*}{} &
% \multicolumn{3}{c}{Cross-Task} &
% \multicolumn{3}{c}{Cross-Website} &
% \multicolumn{3}{c}{Cross-Domain} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
& Offline\textsubscript{0}& Offline\textsubscript{1} & Online \\
\midrule
FLAN-T5-XL&\num{3.33}&\num{20.0}&   \num{28.6}\\
GPT4 &\num{1.11}&\num{12.2}&\num{21.8}   \\
LMM2Web\textsubscript{Human} &&&\num{54.5}\\
LMM2Web\textsubscript{Choices} &\num{4.45}&\num{14.45}&\\

\bottomrule
\end{tabular}
\vspace{-5pt}
%\captionsetup{width=0.95\textwidth} 
\caption{Whole task success rate tested in both static environment (off) and online environment (on). Off-0 and Off-1 refers to tolerance for error by zero or one action step.}
\label{tab:online_evaluation}
\end{table}

% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|ccc|ccc|ccc|}
% \hline
%   & Cross-Task & \multicolumn{3}{c|}{Cross-Website} & \multicolumn{3}{c|}{Cross-Domain}  \\
%  & Ele. Acc & Op. F1 & Step SR & Ele. Acc & Op. F1 & Step SR  & Ele. Acc & Op. F1 & Step SR\\
% \hline
% MindAct-XL~\cite{deng2023mind2web} & 55.1&75.7&52.0  &42.0&65.2&38.9  &42.1&66.5&39.6\\
% HTML-T5-XL~\cite{Gur2023ARW}  &76.4&78.8&71.5  &68.4&71.0&62.2  &73.0&75.6&67.1\\
% WebGUM-XL~\cite{Furuta2023MultimodalWN}  &70.8&75.9&64.9   &69.1&75.3&62.5  &73.1&77.7&66.7\\
% \hline
% GPT-3.5 &  & &    &&&  &&&\\
% GPT-4-Text&  &    &  &&&  &&&\\
% EXP2 &  &  &   &10.53&&  &&&\\
% EXP4 & 53.08 & 90.69 & 50.64   &46.01&&  &&&\\
% EXP3 &  &  &    &&&  &&&\\
% Human Refer& 72.84 &    &  &&&  &&&\\
% \hline
% \end{tabular}
% \caption{Perfomance on GPT-4Vision with different choice style. EXP4 (Only Text) is the original method proposed in MindAct~\cite{deng2023mind2web} using GPT4 Text-Only. We group methods into two groups: SL for supervised training or fine-tuning and ICL for in-context learning.
% }
% \end{table*}
% \label{tab:online_evaluation}


==> sec/related_works.tex <==
\section{Related Work}
\subsection{Large Multimodal Models}
The development of LMMs has been characterized by large-scale image-text pretraining to achieve in-context learning capabilities~\cite{Wang2021SimVLMSV, Wang2022GITAG, Chen2022PaLIAJ, Chen2023PaLIXOS, Li2023BLIP2BL, Alayrac2022FlamingoAV, Driess2023PaLMEAE, Monajatipoor2023MetaVLTI, Aghajanyan2022CM3AC, Yu2023ScalingAM}. Further work focuses on improving instruction following~\cite{Ouyang2022TrainingLM, Peng2023InstructionTW} capabilities with curated multimodal instruction-following data~\cite{Zhu2023MiniGPT4EV, Dai2023InstructBLIPTG, Liu2023VisualIT} and alignment with reinforcement learning from human feedback~\cite{Sun2023AligningLM}.
% Flamingo integrates a pretrained CLIP image encoder with large language models (LLMs) using gated cross-attention blocks, showcasing multimodal in-context learning capabilities. Similarly, BLIP-2 employs a Q-Former to align visual and textual embeddings, integrating these with LLMs via a fully connected layer. 
% Instruction tuning, as explored in~\cite{Ouyang2022TrainingLM, Peng2023InstructionTW}, further enhances a model's capacity to follow instructions. MiniGPT-4~\cite{Zhu2023MiniGPT4EV} and InstructBLIP~\cite{Dai2023InstructBLIPTG} leverage the Q-Former architecture and are fine-tuned with specially curated instruction-following data. LLaVa~\cite{Liu2023VisualIT} projects the outputs of its visual encoder to the LLM using a trainable fully connected layer, with fine-tuning conducted using the LLaVa-150K instruction dataset.
\gptv~\cite{OpenAI2023GPT4TR} and Gemini~\cite{Anil2023GeminiAF} represent significant progress in LMMs. Several studies~\cite{Akter2023AnIL, OpenAI2023GPT4TR, Yang2023TheDO, Zhang2023GPT4VisionAA, Yang2023SetofMarkPU, Yan2023GPT4VIW} have highlighted their remarkable multimodal capabilities, emphasizing the advanced and versatile integration of visual and language reasoning abilities. Their performance on a series of benchmarks~\cite{Kazemzadeh2014ReferItGameRT, Goyal2016MakingTV, Hendrycks2020MeasuringMM, Saikh2022ScienceQAAN, Lu2022LearnTE, Zhong2023AGIEvalAH, Yue2023MMMUAM} also showcases remarkable capabilities on vision-and-language understanding and reasoning.
% The evolution of large multimodal models (LMMs) has been characterized by significant progress in large-scale image-text pertaining, including SimVLM~\cite{Wang2021SimVLMSV}, GIT~\cite{Wang2022GITAG}, PaLI~\cite{Chen2022PaLIAJ}, PaLI-X~\cite{Chen2023PaLIXOS}, BLIP-2~\cite{Li2023BLIP2BL}, Flamingo~\cite{Alayrac2022FlamingoAV}, PaLM-E~\cite{Driess2023PaLMEAE}, MetaVL~\cite{Monajatipoor2023MetaVLTI}, CM3~\cite{Aghajanyan2022CM3AC}, and CM3Leon~\cite{Yu2023ScalingAM}. 
Although open-sourced models still exhibit a performance gap with \gptv, they have the advantages of controllability and ease of fine-tuning for various applications. For example, in CogAgent~\cite{Hong2023CogAgentAV}, LMMs are fine-tuned on HTML and screenshot image pairs to enhance webpage understanding ability and further enhanced with an image encoder for high-resolution image details. Ferret~\cite{You2023FerretRA} is finetuned to allow visual referring and grounding. 

\subsection{Web Agent}
Driven by the vision of achieving a seamless human-web interaction, considerable initiatives have been invested in web agents that can understand language instruction and complete tasks on the web. Significant efforts have been invested in building benchmarks for web agents with simplified environment simulation~\cite{liu2018reinforcement, Shi2017WorldOB, Mazumder2020FLINAF, Yao2022WebShopTS}. WebArena~\cite{Zhou2023WebArenaAR} creates website simulations in the sandbox from four popular categories with functionality and data mimicking their real-world equivalents. Mind2Web~\cite{deng2023mind2web} instead provides environments in diverse domains, websites, and various tasks on real-world websites by dumping webpages from live websites along with action trajectory annotation. Similar benchmarks have also been proposed for mobile UI automation~\cite{Burns2022ADF, Li2020MappingNL, Sun2022METAGUITM}. To improve web agent performance, WebAgent~\cite{Gur2023ARW} pretrains a T5 model on HTML data and performs instruction tuning to enable long HTML document summarization and action planning. Pix2Act~\cite{Shaw2023FromPT} solely replies on pixel-based screenshots as input by parsing them to simplified HTML with Pix2Struct~\cite{Lee2022Pix2StructSP}. WebGUM~\cite{Furuta2023MultimodalWN} enables web agents to observe both HTML and the rendered screenshot by fine-tuning LMM with a large multimodal corpus for web agents. CogAgent~\cite{Hong2023CogAgentAV} further improves with a high-resolution image encoder to enable the agent to recognize small webpage elements and texts. In a concurrent work~\cite {Yan2023GPT4VIW}, \gptv\ exhibits strong performance on mobile UI understanding, which is much simpler than the desktop websites we study.


\subsection{Visual Grounding}
While LMMs, especially \gptv\ and Gemini, have achieved remarkable vision-language understanding capabilities, they still face challenges in fine-grained visual grounding. Various visual prompting methods have been proposed to augment \gptv's image detail grounding ability. Typically, these methods involve overlaying visual marks onto images, facilitating the model's reference and grounding to specific regions. Various types of visual marks have been explored, such as red circles~\cite{Shtedritski2023WhatDC}, mask areas~\cite{Yang2023FineGrainedVP}, and combinations of circles, arrows, and hand drawings~\cite{Yang2023TheDO}. SoM~\cite{Yang2023SetofMarkPU} involves segmenting the image into semantically meaningful regions and overlaying an array of visual marks like numbers, alphabets, masks, or bounding boxes.
Fine-tuning vision-language models with image-annotated data has been shown to be effective. Kosmos-2~\cite{Peng2023Kosmos2GM} represents bounding box locations through textual location tokens. BuboGPT~\cite{Zhao2023BuboGPTEV} extract entities and find corresponding masks for objects in the image. Shikra~\cite{Chen2023ShikraUM} handles image detail referring and grounding by applying spatial coordinates as text tokens in inputs and outputs, respectively. Ferret~\cite{You2023FerretRA} represents regions with both discrete coordinates and continuous features along with a spatial-aware visual sampler to handle diverse spatial characteristics across various shapes. 





==> sec/upper_bound.tex <==
% \section{Potential of GPT4-V as Web Agent}
% \label{sec:upper_bound}

% \boyuan{Merge with Section 4}

% The performance of GPT-4V in web navigation depends on two critical aspects:

% % \textbf{Action Generation} During each step of action generation, GPT4-Vision initially produces a description for the subsequent action. This description encompasses both a high-level strategy and detailed, low-level steps. Mostly, these steps will be preceded by intermediate thoughts. The quality of generation at this stage represents the upper limit of the model's capability in web navigation tasks. In Section~\ref{sec:upper_bound}, we implement human annotation to manually determine whether the generated intermediate thoughts and action descriptions adequately capture the essence of the intended target element and action.

% \textbf{Action Generation:} At each stage of action generation, GPT-4V first generates a detailed action plan. This plan comprises a strategic overview followed by specific, granular steps, often interspersed with intermediate reasoning. The quality of these initial generations sets the benchmark for the model’s proficiency in web navigation tasks. 
% % As detailed in Section~\ref{sec:upper_bound}, we employ human evaluators to assess whether the intermediate thoughts and action plans effectively encapsulate the core elements of the intended web tasks.

% % first generates a detailed action plan. This plan comprises a strategic overview followed by specific, granular steps, often interspersed with intermediate reasoning. The caliber of these initial generations sets the benchmark for the model’s proficiency in web navigation tasks. 
% % As detailed in Section~\ref{sec:upper_bound}, we employ human evaluators to assess whether the intermediate thoughts and action plans effectively encapsulate the core elements of the intended web tasks.

% \textbf{Element Referring:} Generating an accurate and detailed action plan is only the first step of the challenge. Effective web navigation requires precise identification of and interaction with specific webpage elements. Subsequent to action generation, the model needs to refer to a exact element on the webpage. The methods for this phase are further explored in Section~\ref{sec:referring}.


% In this section, we aim to explore the model's capabilities under the assumption of an optimal element-referring method, thus identifying a performance upper bound for GPT4-Vision on web navigation tasks.

% \subsection{Potential}

% Several challenges and explorations exist to leverage vision-language models for web navigation tasks: (1) How to embed the agent to the web environment presented through screenshot image; (2) Referring to the specific webpage element for execution. 

% \subsection{Human Evaluation}
% \label{exp:human_eval}
% To evaluate GPT-4V's performance cap, we first prompt the model to directly generate descriptions about next step action without constraints of the output format, which allows humans to extract information about the target element, the operation, and any operational values associated with it. 

% In the prompts, we direct the model  to imitate a human navigating the web given a screenshot. We first explicitly  instruct the model to analyze the webpage and previous steps with the screenshot. Then we ask the model to generate an answer of the target element and the corresponding operation. The description is instructed to be precise, detailed and identifiable to help identify and locate the target element.

% % \boyu{[Boyu's Comment: The prompt description is not very identical to our prompts.]}

% % \boyu{[Boyu's TODO: Edit the explanation of the prompts]}

% % \paragraph{Human Annotation}
% % We invite human annotators to label if the generated next step action description contains valid and sufficient information to derive the target webpage element, operation, and operation value.  This assessment provides a benchmark for the model's potential. 
% Human annotators are tasked with determining whether the generated action descriptions contain adequate and valid information to derive the target webpage element, operation, and operational values. This evaluation serves as a metric for the model’s potential in web-based tasks. We perform two-way annotation to label scores for each action, resulting in a Cohen's Kappa Coefficient~\cite{McHugh2012InterraterRT} of @placeholder, denoting a high/medium/low agreement level among annotators. Our results, as illustrated in Figure~\ref{tab:main}, reveal an element accuracy rate of \num{84.9}\%, significantly surpassing existing methods across all evaluated categories.

